A Type System for Julia

The Julia programming language was designed to fill the needs of scientific computing by combining the benefits of productivity and performance languages. Julia allows users to write untyped scripts easily without needing to worry about many implementation details, as do other productivity languages. If one just wants to get the work done-regardless of how efficient or general the program might be, such a paradigm is ideal. Simultaneously, Julia also allows library developers to write efficient generic code that can run as fast as implementations in performance languages such as C or Fortran. This combination of user-facing ease and library developer-facing performance has proven quite attractive, and the language has increasing adoption. With adoption comes combinatorial challenges to correctness. Multiple dispatch -- Julia's key mechanism for abstraction -- allows many libraries to compose "out of the box." However, it creates bugs where one library's requirements do not match what another provides. Typing could address this at the cost of Julia's flexibility for scripting. I developed a "best of both worlds" solution: gradual typing for Julia. My system forms the core of a gradual type system for Julia, laying the foundation for improving the correctness of Julia programs while not getting in the way of script writers. My framework allows methods to be individually typed or untyped, allowing users to write untyped code that interacts with typed library code and vice versa. Typed methods then get a soundness guarantee that is robust in the presence of both dynamically typed code and dynamically generated definitions. I additionally describe protocols, a mechanism for typing abstraction over concrete implementation that accommodates one common pattern in Julia libraries, and describe its implementation into my typed Julia framework.

==> CHANGES <==
Changes in version 4.2 (September 2015)
o Fixed issue between titlesec and tocloft regarding
  part numbering in the ToC (classicthesis.sty). 
	Thanks to Enrico Gregorio and Henri Menke.
o Fixed bug with colored lines and graffiti 
  (classicthesis.sty). Thanks to Enrico Gregorio and
  Stefano Bragaglia for the fix! (Also switched
  graffiti from \slshape to \itshape.)
o Changed \vspace*{8ex} to \vspace{8ex} (Contents.tex)	
o Moved \cleardoublepage from end of Contents.tex 
  to appropriate position in ClassicThesis.tex
o \bflabel of acronym package removed, as it was 
  removed from acronym package and caused errors.
  Now set \aclabelfont to \acsfont for consistency.
o Converted major files to UTF-8 (thanks to Jörn Hees)
  (Bibliography.bib excluded for now as BibTeX cannot
  handle UTF-8)
o Added support for BibLaTeX in 
  classicthesis-config.tex and Bibliography.tex
	(thanks to Jörn Hees).
	For LyX we will have a work-around for testing.
o Added an example for one's own publication list
  (via BibLaTeX) in Publications.tex (renamed from 
	Publication.tex)
o Replaced/updated scrpage2 with scrlayer-scrpage 
  in classicthesis.sty (thanks to Ivo Pletìkosić).
X Worked on Appendix case with floatperchapter 
  (works for captions but not for references so far)
	Thanks to Claus Lahiri and Clemens Niederberger 
	for their help on this.
	[REMOVED DUE TO OTHER PROBLEMS, SEE ISSUE #82]	
X Removed fixltx2e from classicthesis-config.tex and
  have classicthesis.sty use or emulate the latest 
	LaTeX kernel via latexrelease (option: latest)
  (thanks to Jörn Hees).
	[REMOVED AS IT IS NOT AVAILABLE IN MANY 
	DISTRIBUTIONS, SEE ISSUE #107]
	
Changes in version 4.1 (August 2012)
o Working towards XeLaTeX support:
	- "ifxetex" package for checking whether
	  XeTeX is in use (classicthesis.sty)
	- Adjusted part, chapter, and tocEntry 
	- Thanks to Joerg Weber for his ideas and code
	- Option "pdfspacing" does not work for XeTeX
	  and is disabled when XeTeX is running
	  (maybe implement spacing with fontspec later)
o Load additional packages in order to 
  reduce warnings (classicthesis-config.tex)
	- "textcomp" to fix warnings with missing font 
	  shapes
	- "scrhack" to fix warnings when using KOMA 
	  with listings package  
o Replaced \mathrm-command with \textrm-command
  (Chapter03.tex)

Changes in version 4.0 (December 2011)
o Due to lots of issues and complaints, 
  classicthesis-preamble.sty is replaced by 
  classicthesis-config.tex (which is cleaner,
  nicer, better, etc. than before!)
o No per-chapter-numbering also for equations 
  (classicthesis.sty and Chapter03.tex)
o classicthesis.sty now also works without the 
  KOMA-classes (scrbook, scrartcl, etc.):
	- This affects the text body shape, where the
	  package "typearea" is always loaded in order 
	  to use \areaset
	- And affects the layout of footnotes where the 
	  package "footmisc" is loaded otherwise
	  (not 100\% identical look-and-feel but OK)
o Help for using spanish babel with classicthesis 
  (classicthesis-config.tex)
o Note about pdfsync issues with graffiti 
  (Chapter01.tex)
o Minor clean-up of comments and duplicate lines 
  (classicthesis.sty)
o Adjusted the colophon text (Colophon.tex)
o Increased space for labels in the LoF, LoT, LoL
o Included version information on the title page and
  in the drafting and final version information 
  (classicthesis.sty and Titlepage.tex)

Changes in version 3.0 (June 2011)
o There have been some major changes in order to port 
  classicthesis to LyX easily. See below for details.
  Special thanks go to Ivo Pletikosi\'c for all his 
  hard work he put into this project!
o Changes in ClassicThesis.tex:
	- Redundant fleqn removed from documentclass options 
	 (will be set by amsmath package in preamble)
	- KOMA adjustments for documentclass: 
	  fontsize=11pt,paper=14
	- Moved language options into documentclass due to LyX
	  issues with babel
o Changes in classicthesis.sty:
	- Removed bcor from \areaset command so that it can
	  be set via \documentclass option (BCOR=)
	- New \ctparttext command for putting preamble text
	  after part titles (see ClassicThesis.tex for examples)
	- \graffito command now also available as original
	  \marginpar (backward compatibility is enabled)
	- Chapter number in margin done with \oldmarginpar
o Changes to classicthesis-preamble.sty:
  - Fixed autoref for subfigures (see Chapter 2 for example)
  - Fixed issues with redefining autoref strings (for
      different languages)
	- Now contains all configuration information, such as
	  the title, your name etc.
	- This package now also loads classicthesis.sty, change
	  the options classicthesis to be loaded with here  
	- Package inputenc now loaded with latin9 option 
	- Package listings now also loaded here
	- Now safer package loading regarding options by
	  using \PassOptionsToPackage command extensively
	- Inserted new string for \mySubtitle
o Changes in Titlepage.tex and Titleback.tex because of new 
  string \mySubtitle
o Changed a lot of the documentation, e.g., in Chapter01.tex

Changes in version 2.9 (January 2011)
o Fixed onlytext euler font for MinionPro font (in 
  classicthesis.sty)
o Option "listsseparated" deprecated, because it led to some
  strange side-effects (in classicthesis.sty)
o Changed default font size to 11pt (in ClassicThesis.tex) and
  adjusted text block size accordingly (in classicthesis.sty)
o Fixed bug with backward compatibility regarding old commands
  \myChapter and \myPart in classicthesis.sty
o New option "floatperchapter" for classicthesis.sty, removed 
  all code for that from classicthesis-ldpkg.sty
o Removed "nochapters" option from classicthesis-ldpkg.sty
o Removed redundant loading of listings package (in
  classicthesis-ldpkg.sty)
o Fixed some headline bug in example classicthesis-book.tex
o Fixed a bug when using parts with plain latex as in example
  classicthesis-book.tex (in classicthesis.sty)

Changes in version 2.8 (March/May 2010)
o Fixed serious \graffito bug in classicthesis.sty
  (thanks to Lorenzo Pantieri and Enrico Gregorio)
o Included backward compatibility regarding old commands
  \myChapter and \myPart in classicthesis.sty
o Fixed drafting issues (draft information not shown at all)
  caused by wrong code for listings and listsseparated options
  in classicthesis.sty 

Changes in version 2.7 (February 2010, cumulative release)
o Removed option for classicthesis-ldpkg.sty: nobackref 
  Introduced instead option "backref" for consistency
  which works the other way (no backrefs by default)
  
Changes in version 2.6.2 (January 2010, released as beta)
o New option for classicthesis-ldpkg.sty: nobackref 
  (removes links to cited page in bibliography)
o Fixed some spacing issues for LoF, LoT, LoL with option
  "listsseparated" (in classicthesis.sty)

Changes in version 2.6.1 (October 2009, released as beta)
o Removed \myChapter and \myPart, you can now use the regular
  \chapter and \part commands (in classicthesis.sty)
  (thanks to Hinrich Harms for this)
o Fixed used KOMA-options: numbers=noenddot, cleardoublepage=empty
  (in ClassicThesis.tex)
o Included hack to use citations in float environments, will 
  be fixed with caption package version 3.2 (in classicthesis.sty)
o Included some font and text area fine-tuning code 
  (in ClassicThesis.tex)
o Some testing with Libertine font (classicthesis-book.tex)
o Fixed numbering of listings used in different chapters
  (in ClassicThesis.tex, classicthesis.sty, classicthesis-ldpkg.sty)
o Spacing between listings in different chapters and after List 
  of Listings header fixed (in classicthesis.sty)
o Increased \newnumberwidth to sizeof(999) which is better for 
  documents with more than 99 pages (in classicthesis.sty)
o New option for classicthesis.sty: manychapters
    
Changes in version 2.6 (August 2009)
o Centered the title page with the addmargin environment
  (thanks to Nicolas Repp for the hint)
o Fixed header for page two of Table of Contents (with 3 
  or more pages) (in Contents.tex)
o Added numbering of \subsubsection (in Contents.tex)
o Added correct Table of Contents entries for \subsubsection
  (in classicthesis.sty)
o Added printonlyused option to loading acronym package
  (in classicthesis-ldpkg.sty)
o Some code for "clean" hyperlinks (w/o color and w/o boxes)
o Minor fix for \graffito (in classicthesis.sty)

Changes in version 2.5.1 (May 2009, released as beta)
o New option for classicthesis.sty: dottedtoc
  (Refer to the manual for more information.)
o New option for classicthesis.sty: listings
  (Refer to the manual for more information.)
  (Credit + thanks to Prof. Enrico Gregorio)
o Minor clean-up and bug-fixing

Changes in version 2.5 (October 2008, cumulative release)
o Increased text-width for better page layout (experimental)
o Cumulative release, some minor clean-up and bug-fixing

Changes in version 2.4.{1--3} (February and April 2008,
released as betas)
o Switched back to "obsolete" KOMA options due to 
  compatibility issues on some installations
o Increased robustness of \cauthor command in 
  classicthesis-ldpk.sty
o Spacing fix for \sectionmark (in classicthesis.sty) 
o Made Booleans private (in classicthesis.sty)
o Acronyms header for long acronym lists (in Contents.tex)
o Moved "amsmath" package from classicthesis.sty to
  ClassicThesis.tex
o "MinionPro" package now loaded with "mathlf" option
  instead of "osf" option (in classicthesis.sty)
o Fixed issue with contents headings (in classicthesis.sty
  and in Contents.tex)
o Thanks to Lorenzo

Changes in version 2.3 (November 2007)
o Fixed serious bug with \myChapter command (using plain 
  LaTeX)
o Removed hypcap package from classicthesis-ldpkg.sty and
  placeins package from classicthesis.sty. Put both into
  ClassicThesis.tex for finer end-user control
o Removed obsolete KOMA options from ClassicThesis.tex
o Option "subfigure" deprecated, replaced by "subfig" (in 
  classicthesis.sty)
o Inserted some mechanisms to detect whether subfig(ure) 
  package was loaded or not (in classicthesis.sty)
o Inserted some mechanism to detect whether classicthesis
  packackage was loaded or not (in classicthesis-ldpkg.sty)
o Moved "headlines" code block a bit up in 
  classicthesis.sty (seemed to cause problems with new
  KOMA-Script classes)
o Removed accidental "natbib" from classicthesis-ldpkg.sty  
o Some fine-tuning in (Dirty)Titlepage.tex
o Thanks to Lorenzo and Denis! :-)

Changes in version 2.2 (October 2007)
o \myChapter and \myPart now take an optional argument
  just as the regular \part and \chapter commands
o Did some minor changes to classicthesis-book.tex
  so it's a better example
o Inserted some \cleardoublepage before \myPart 
  occurences to avoid pdfbookmark problems
o Introduced some general typographic fine-tuning
  (linespread, penalties, etc.)
o Did some fine-tuning of the \graffito command

Changes in version 2.1 (July 2007)
o Removed duplicate xcolor package call from 
  classicthesis-ldpkg.sty and shifed some color
  definitions around
o Removed re-definition of \ttdefault

Changes in version 2.0 (June 2007, cumulative release)
o Better setup of the list of acronyms 
  (in classicthesis-ldpkg.sty)
o Using KOMA option footinclude in ClassicThesis.tex
  (text block sizes are adjusted to this)
o New option for classicthesis.sty: minionpro
o New option for classicthesis.sty: minionprospacing
o New option for classicthesis.sty: pdfspacing
  (Refer to the manual for more information.)

Changes in version 1.7 (May 2007, not released separately)
o Removed \graphicspath from ClassicThesis.tex
o Use the nag package to ensure "compliance"
o Switched from ccaption to caption in classicthesis-ldpkg.sty
  (setup via \captionsetup in ClassicThesis.tex)
o Switched from subfigure to subfig in classicthesis-ldpkg.sty
o Removed obsolete "usenames" option from loading xcolor package
o Noticed problem with \thelstlisting on some installations
  (commented out in classicthesis-ldpkg.sty)
o Noticed problem with some hyperlinks on some installations
  (could not determine cause)

Changes in version 1.6 (April 2007, not released separately)
o Included greetings to Lorenzo Pantieri for many very useful
  suggestions
o Introduced new commands in classicthesis-ldpkg.sty to make
  adaptation of backrefs to different languages easier
   - \backrefnotcitedstring (ref is not cited)
   - \backrefcitedsinglestring (ref is cited on one page)
   - \backrefcitedmultistring (ref is cited on multiple pages)
o Removed ellipsis package from classicthesis-ldpkg.sty due to 
  some undesired results for some users
o Removed the following packages from classicthesis-ldpkg.sty as 
  these seem to require changes to their options from most users:
  inputenc, babel, natbib (now in ClassicThesis.tex)
o New option for classicthesis-ldpkg.sty: nochapters
  Use the package with classes that do not have chapter divisions 

Changes in version 1.5 (April 2007, not released separately)
o Fixed some bugs to use classicthesis.sty for article layout
o Inserted some info/warnings when using nochapter/parts
o Extended the manual: examples for using classicthesis.sty for
  other projects than a thesis (source available in folder
  "Examples")
o Some minor adjustments in classicthesis-ldpkg.sty
o Fixed some spelling mistakes

Changes in version 1.4.2 (March 2007)
o Renamed loadpackages.sty to classicthesis-ldpkg.sty due to
  TeX Live package tree issues

Changes in version 1.4.1 (March 2007)
o Fixed some wording concerning the license :-o
o Added fixltx2e and ellipsis packages to to loadpackages.sty to correct
  some minor glitches
o Fixed and changed some things about ToC entries of parts
o Some minor bug fixes

Changes in version 1.4 (January 2007)
o Replaced \lineheight with \baselineskip in classicthesis.sty
o Removed obsolete "usenames" option from xcolor package (classicthesis.sty)
o Now classicthesis.sty processes the global a5paper option and adjusts 
  the layout accordingly (experimental!)

Changes in version 1.3.1 (August 2006)
o Urgent bug concerning ToC spacing etc. fixed

Changes in version 1.3 (August 2006) 
o New option for classicthesis.sty: parts
  Turn this on if you use Part divisions. It fine-tunes the ToC and
  adds support for Part division via \myPart{} (cf. \myChapter{})
  (The style of this feature is preliminary, any suggestions?!)
o New option for classicthesis.sty: eulermath
  Uses the awesome Euler fonts for math (Palatino fonts are default).
o Added mparhack package to loadpackages.sty to get the graffiti right
o Added a hint to loadpackages.sty on how to typeset the List of 
  Listings consistently with classicthesis
o Some minor fine-tuning of typographic details
o Collaboration with babel package improved (now easier to use
  with other languages than English)
o Added appropriate textwidth values for 11pt Palatino and Minion
  (See comments near \areaset in classicthesis.sty)
o Note: There is a problem with the case of math text in part-, 
  chapter-, and section titles and I have no clue how to fix this 
  (either the case or the spacing breaks). So far, I chose the case. :-(

Changes in version 1.2 (June 2006)
o Setup a little postcard collection: http://postcards.miede.de
o Changed stupid spelling mistake: "A Homage" => "An Homage" D'oh!
o New option for classicthesis.sty: nochapters
  Allows to use the look-and-feel with classes that do not use chapters.
o New option for classicthesis.sty: beramono
  Loads Bera Mono as typewriter font. (Default = no typewriter font.)
o Included list of files, see LISTOFFILES.  

Changes in version 1.1 (May 2006)
o classicthesis.sty now stand-alone and usable w/o whole bundle!
o classicthesis.sty compatible with both LaTeX and PDFLaTeX
  Note: this is only true for classicthesis.sty, not the whole bundle.
o New option for classicthesis.sty: subfigure
  Tells the style to add the respective option when loading tocloft.
o Now loading microtype package w/o options (classicthesis.sty)
o Fixed overfull hbox warnings for ToC entries (classicthesis.sty)
o No longer depending on a particular caption package (classicthesis.sty)
o Layout for subsubsections provided (classicthesis.sty)
o PDF opens on title page (ClassicThesis.[tex|pdf])
o Files are a bit more "ASCII-friendly" (all)
o Note: Thanks to all the folks who already sent me a postcard! :-)

Version 1.0 (March 2006)
o First public release

==> Chapters/Chapter01.tex <==
%************************************************
\chapter{Introduction}\label{ch:introduction}
%************************************************

Computer programming languages provide abstractions for expressing our computational intent. 
Historically, languages have come in one of two flavors. First are productivity languages,
designed to enable rapid and interactive changes to the system at the price of performance, 
facilitating the development of software systems. 
Second, performance languages are designed to allow users to write efficient code at the cost
of higher development effort. Increasing productivity often entails relinquishing control
over certain aspects of the computation and delaying some decisions which both typically
degrade performance. Of course, there are many dimensions to modern computer
languages, and the distinction between the two flavors can be blurred.

This thesis focuses on a feature that often distinguishes the two language
flavors: static type checking. A statically type-checkable language can be
augmented with a tool, a type checker, that catches potential programming
errors before the program is run.  Furthermore, a program that has been
checked can often be more efficiently compiled as the compiler is able to rely
on type information when making optimization decisions. Two reasons hold many
productivity languages back from static type checking, however. First, these
languages often include features that are inherently difficult to check before
execution of the program. Second, enforcing a static type system renders
programs more rigid, inhibiting the kind of exploratory programming that these
languages are popular for.

My goal is to extend a productivity language with a static type system, but to
do so in a non-invasive way. Statically typed code should coexist with untyped
code.  With such a system programmers are able to pick whether to write code
that will be  checked or to ignore the type system when it gets in the way.
The ability to choose whether one wants checking or not allows developers of
large systems to statically check their code while still enabling script
writers to use said systems without  needing to worry about satisfying the
type checker. Choice then allows the benefits of both productivity and
performance languages.

A number of criteria should hold in order to reap the benefits of static
checking. First, there should be a clear and well-understood guarantee about
which errors can not occur in the checked parts of the code. Additionally, no
(or very few) performance regressions should occur due to typing. Finally, it should
be possible to opt-in or opt-out of typing so as to provide the requisite agency
to the developer.

\paragraph{Julia.} I have chosen the Julia language as my concrete target
language. Julia is a relatively young system with a combination of
productivity and performance features. It was developed at MIT in the last
decade by a small academic team,  and has since become increasingly popular
within scientific computing.  Today, Julia is used in applications ranging
from climactic modeling to numerical optimization, with a steadily growing
user base.  There are flies in the adoption and scale ointment, however. 

Julia libraries have grown to be of considerable size, exceeding hundreds of
thousands of lines in some cases. The developers and users of these libraries
are frustrated by simple type bugs, unreliability, and confusing error
messages. One selling point of Julia is that it allows easy composition of large
libraries; however, when one composes libraries, one also composes their bugs. 
Composing libraries causes the potential for error to expand combinatorially for
each inter-library interaction begets the opportunity for some new and exciting
edge case to spring up. Julia, presently, has no formalized mechanism for checking
or even describing these interactions. Consequently, it has gained some notoriety
for being buggy around these very interactions\footnote{\url{https://yuri.is/not-julia/}, \url{https://github.com/JuliaStats/Distances.jl/issues/201}}.

Types are the standard answer for building abstraction over implementation.
Abstract types, in particular, allow specification of some generic behavior
that should hold for some specific instantiation of the type. Typing most
untyped languages is difficult, though, for a notion of type must be added
on top of the existing language concept. Julia is different.

In spite of being an untyped productivity language, Julia programs are full of
types. Almost all methods in the most popular Julia libraries have at least on
type annotated argument and the overwhelming majority are fully
typed~\cite{oopsla18a}. Moreover, most struct fields carry a type annotation.
If Julia is untyped, why should programmers write all of these types?

Julia programmers write types because Julia's runtime uses them. Julia's
implementation relies on types for two key applications: First, type annotated
field writes are checked. These checks are performed each time the field is
updated during program execution. Stored values can therefore be relied upon
to be type-correct. In turn, this correctness guarantee lets compiled code
safely read from typed fields. Second, types are used for dispatch, wherein
Julia decides what implementation should be invoked from a given call site.
Julia uses a mechanism called multiple dispatch to decide what method to
invoke. Each Julia function can have multiple implementations, or methods,
with each method having differently type annotated arguments. Julia will
dynamically dispatch function invocations to the method with the most
applicable type annotations. Julia therefore dynamically guarantees that
arguments will be of their declared types.

These guarantees mean little, however, when they are not exposed to the
programmer. As the scale of the Julia ecosystem increases, so does the
likelihood that some argument, somewhere, is misused. It does not matter if
the argument is a member of the statically-declared type annotation if the
method body calls a function on it that does not exist. Thus, there may be
cases where no applicable method exists for some call site. Only when code is
exercised are these errors discovered, but not all code is exercised with all
possible types during testing. Moreover, Julia's design allows users to
introduce new types and thread them through existing code, further creating
edge cases whereby invocations can go wrong.  As a result, bugs in Julia code
can hide from developers, hidden under a thin layer of passing tests and
faulty unstated assumptions, only to jump out when a user is least expecting
it. A static type system can help identify these issues ahead of time,
improving reliability of Julia code and easing development.

\paragraph{Research Questions.} 
This thesis answers several questions that stand on the way to statically typed Julia. My goal is
to show the basic feasibility of a type system for Julia and develop a framework within which the
key obstacles for typing Julia can be found and solved.

\begin{enumerate}
%\item \emph{What is the landscape of gradual type systems for object-based languages?}
%    Mixing typed and untyped code has been the focus of extensive study in the context of gradual typing. Which of the many approaches
%    is the right one for Julia?
\item \emph{What is Julia's notion of subtyping?} 
    In order to statically type Julia one must interact with Julia's type system. In turn, Julia's type system (and execution model)
    depends heavily on Julia's notation of subtyping. Every step of method selection during dispatch depends on subtyping, for example.
    How does Julia's subtyping work, can it be used as part of a static type system, and can the system accommodate all of its features?
\item \emph{Can performance be preserved in the face of challenging language features?}
    Some past approaches to gradual typing imposed huge performance impacts, particularly for highly dynamic code. Can a type system
    offer both low overhead and soundness while still supporting key Julia language features like dynamic code generation?
\item \emph{Can we implement a partial type checker for Julia?} Can a idiomatic static type system for Julia be built?
    In particular, is there a gradual type system system that supports existing design patterns and idioms alongside dynamically typed code, all while retaining performance?
\end{enumerate}


\section{Motivation}

One of Julia's selling points is the composition of libraries using multiple dispatch.
Suppose we wanted to differentiate the function \c{f(x)=x*sin(x)+x*cos(x)} about \c{5}. 
We could differentiate the function's implementation on paper, but if \c{f} was even slightly complex this becomes impractical. 
We could also use finite differencing, but this is imprecise. 
In Julia, however, computing the derivative is as simple as:
\begin{jllisting}
 > using ForwardDiff
 > ForwardDiff.derivative(f, 5)
 5.537670211431911
\end{jllisting}
The library works by replacing the argument of \c{f} with a dual number. 
The dual number extends every operation on numbers to operate on the stored derivative value.

Consider the operation \c{x+y}, an invocation of the function \c{+} on the variables \c{x} and \c{y}. 
To evaluate this simple addition, Julia must select which method to invoke out of over 190 options:
\begin{jllisting}
# 190 methods for generic function "+":
[1] +(x::T, y::T) where T<:Union{Int128, Int16, Int32, Int64, Int8, UInt128, UInt16, UInt32, UInt64, UInt8} in Base
[2] +(c::Union{UInt16, UInt32, UInt8}, x::BigInt) in Base.GM
[3] +(c::Union{Int16, Int32, Int8}, x::BigInt) in Base.GMP
[4] +(c::Union{UInt16, UInt32, UInt8}, x::BigFloat) in Base.MPFR
[5] +(c::Union{Int16, Int32, Int8}, x::BigFloat) in Base.MPFR
...
\end{jllisting}
The selection is based on two criteria. First, the dispatch algorithm selects methods that are \emph{applicable}, 
in other word, methods whose argument type annotations include the types of the actual values provided.
Second, the dispatch algorithm must, out of all applicable methods, find whichever one is the most \emph{specific}, the one that most accurately describes the provided arguments. 
All arguments participate in dispatch; no preference is given to any single argument.

As an example, consider the case where both \c{x} and \c{y} are \c{Int64}. 
The following methods are all \emph{applicable}:
\begin{jllisting}
[1] +(x::T, y::T) where T<:Union{Int128, Int16, Int32, Int64, Int8, UInt128, UInt16, UInt32, UInt64, UInt8} in Base
[2] +(a::Integer, b::Integer) in Base
[3] +(y::Integer, x::Rational) in Base
[4] +(x::T, y::T) where T<:Number in Base
[5] +(x::Number, y::Number) in Base
\end{jllisting}
The algorithm chooses the first of these implementations as when the variable \c{T} is bound to \c{Int64}, the first method describes exactly the arguments at the call site.
All other implementations handle some additional value types, and are thus less specific.

As the number of libraries in the Julia ecosystem increases, errors become more frequent.
Julia relies on undocumented interfaces, of which \jlinl{+} is a member for numeric values.
Programmers expect to be able to add number-like-things, but there is no specification for
either what a number-like-thing is, or what \jlinl{+} actually should do. 

Suppose that instead of using forward differentiation to calculate the derivative of \c{f},
we instead wanted to do it symbolically using computer algebra. We can do this in Julia 
by using the \jlinl{Symbolics} library as follows:
\begin{jllisting}
 > using Symbolics: variable, solve_for
 > x = variable(:x)
 > eqn = f(x)
 x*cos(x) + x*sin(x)
 > Symbolics.derivative(eqn, x)
 x*cos(x) + cos(x) + sin(x) - x*sin(x)
\end{jllisting}
Now, instead of passing a dual number to \jlinl{f} for automatic diferentiation, we pass the symbolic
variable \jlinl{x}.
This symbolic variable accumulates the operations performed on it, constructing an equation describing the computation, which we can then symbolically differentiate. 
This can readily go wrong, however, on a function like \c{g}:
\begin{jllisting}
function g(x) 
   result = 0
   for i=1:x 
     result += i
   end
   return result
end
\end{jllisting}
Symbolically differentiating \c{g} with respect to \c{x} yields the error:
\begin{jllisting}
ERROR: TypeError: non-boolean (Num) used in boolean context
Stacktrace:
 [1] unitrange_last(start::Num, stop::Num)
   @ Base .\range.jl:294
 [2] UnitRange{Num}(start::Num, stop::Num)
   @ Base .\range.jl:287
 [3] Colon
   @ .\range.jl:5 [inlined]
 [4] Colon
   @ .\range.jl:3 [inlined]
 [5] f(x::Num)
   @ Main .\REPL[19]:3
\end{jllisting}
This is an example of where the lack of agreement on what it means to be a number-like-thing bites us.
Here, should all number-like-things be usable as iteration bounds?
The function \c{g} implicitly assumes that yes, numbers should be usable in iteration bound. 
Normal numbers satisfy this unstated assumption, but abstract variables such as those introduced by Symbolics cannot.
Moreover, there is no way to specify that \c{g} takes arguments that can serve as loop bounds.
This fundamental lack of agreement on what it should be possible to do to a number can create unexpected
errors from deep within programs that are difficult to understand; why, in this example, is the error referring to
using a non-boolean as a boolean even though the real issue is that we are trying to bound iteration with an algebraic 
variable? Deep inspection of the library's source code can answer this question, but most programmers would prefer not
to have to do this to identify simple errors of this nature.

My aim is to prevent such errors by enforcing a typing discipline in selected portions of the code.

\subsection{Gradual Typing.}
Julia already performs some amount of type checking. 
Consider the following small Julia program.
As the user provided no type annotations they defaulted to \c{Any}, a type that can be inhabited by any value.
\begin{jllisting}
mutable struct Node
    val
    nxt
end
function insert(list, elem)
    if list isa Void
        return Node(elem, nothing)
    elseif list.val > elem
        return Node(elem, list)
    end
    list.nxt = insert(list.nxt, elem)
    list
end
\end{jllisting}
The implementation needs not perform any checks, but the code tests the type of \c{list} using the \c{isa} operation.
Now, consider this slightly modified version with type annotations.
\begin{jllisting}
mutable struct Node
    val
    nxt :: Union{Node, Void}
end
function insert(::Void, elem)
   return Node(elem, nothing)
end
function insert(list::Node, elem)
    if list.val > elem
        return Node(elem, list)
    end
    list.nxt = insert(list.nxt, elem)
    list
end
\end{jllisting}
Here, Julia will check the type of the first argument of \c{insert}. If the first argument is \c{Void} then the first method is called.
If the type of the first argument is \c{Node} then the second method is called.
Moreover, Julia enforces the type of \c{nxt}; whenever it is assigned, either through object creation or explicit assignment, the runtime ensures
that the value adheres to the declared type.

On the other hand, a value without annotation is assumed to be of type \c{Any}. These values could hold anything and the compiler can make
no assumptions about their contents.

The challenge for mixing code that is statically typed with code that isn't is how to deal with the flow of values annotated as \c{Any}.
My intuition is that right approach is to leverage the existing run-time type checking infrastructure.
For example, in the above code fragment, while it is possible that use of \c{list} is correct, the other argument is used for a comparison.
To type the \c{insert} function one has to require that \c{elem} is a comparable value.
The following would be sufficient, though more restrictive than necessary.
\begin{jllisting}
function insert(list::Node{T}, elem :: T where T <: Number)
    if list.val > elem
        return Node(elem, list)
    end
    list.nxt = insert(list.nxt, elem)
    list
end
\end{jllisting}
This definition is type safe, as \c{Numbers} in the standard library support comparion.
New definitions of Number could be added at any time, however, that do not support comparison or implement it in unexpected ways.
One example is the aforementioned algebraic variables where the result of comparision is not a boolean variable but instead
an algebraic computation.
We will return to this question later in this proposal.

\subsection{Subtyping.}
Julia's type language inlcudes nominal single subtyping as well as union,
parametric invariant existential, and covariant tuple types. Subtyping of
unions and tuples is distributive, including over parametric types, which
Julia augments with the so-called diagonal rule.

In conjunction, Julia's type language features allow users to write highly
specific method signatures. For example, we can write \jlinl{+(::V, ::Diagonal{T, V}) where {T <: Real, V <: Vector{T}}}
to describe a function that adds a vector of real numbers to a diagonal matrix
with a backing array that is a \jlinl{Vector} of precisely the same real number type.
With this power, however, comes decision challenges.

Julia's subtyping relation is inspired by the notion of semantic subtyping,
wherein if every value contained in one type is in another then it is a
subtype. The idea of semantic subtyping is intuitive, but hard to decide, and
thus Julia's subtyping mechanism merely aims to imply semantic subtyping but 
not vice versa. Several language features still make life difficult, though.

Tuples and covariant unions are one example. Checking that \jlinl{A <: B}
entails proving that every element of \jlinl{A} is contained within some
instantiation of \jlinl{B}, either through choices at union types or of type
variable instantaition. We would like the type \jlinl{Tuple{Union{Int,
String}, String}} to be equivalent to  \jlinl{Union{Tuple{Int, String},
Tuple{String, String}}} to achieve the semantic-like intuition. However,
standard approaches directly normalize the union-in-tuple of the first type to
the union-of-tuples in the latter, which can take exponential space. Julia
instead checks that this property holds using a linear space, exponential time
backtracking algorithm that had not previously been used in a subtyping
decision procedure, which I proved was correct and terminating.

Julia's type language is by no means restricted to unions and tuples, however,
making our lives considerably more difficult. In particular, it supports
bounded polymorphism, as the above example of addition implies, which starts
to ring alarm bells. Considerable prior work such
as~\cite{Grigore:2017:JGT:3009837.3009871} identified undecidability in type
systems arising from such quantification. I was able to prove that subtyping
in Julia is undecidable by reduction from System $F_{<:}$~\cite{Pierce92},
showing that type checking in Julia is potentially nonterminating.

While undecidability of subtyping is not fatal for type checking, it (and its
broader impacts on the project) need to be considered in the design of the
static type system. The Julia project aims to eliminate the undecidability,
but in so doing may change the type system. While the most likely avenue for
making this fix is in eliminating a virtually unused feature of the type
system (lower bounds on existential type variables), it  means that the static
type system cannot be attached to any one type language.

I therefore propose a \emph{generic} type system for Julia that abstracts over
the concrete type language. I instead will assume a set of properties about
types (and subtyping), such as correctness with reference to the semantic
definition, and then show that correctness follows assuming that these axioms
hold. This abstraction decouples research on the type system from research on
the type language, allowing independent development on each front.

\subsection{World Age.}
\newcommand{\eval}{\c{eval}\xspace}
\newcommand{\Eval}{\c{Eval}\xspace}

Dynamic programming languages face semantic and performance challenges in the
presence of features, such as \eval, that can inject new code into a running
program. Julia's use of open functions, wherein new methods can be added from
anywhere and anywhen, then creates an obvious problem. Code added by \eval
could, in theory, be invoked from previously-compiled or typechecked call
sites, invalidating all downstream assumptions made before the code was added.
Julia introduces the concept of world age to address this issue.

Julia provides a number of built-in functions for run-time introspection and meta-programming. 
For instance, the methods of any function \c f may be listed using \c{methods(f)}. All the methods are stored in a special data structure, called the  \emph{method table}.  
It is possible to search the method table for methods accepting a given type: for instance, \c{methods(*,(Int,Float64))} will show methods of \c * that accept an integer-float pair.
The \eval function takes an expression object and evaluates it in the global environment of a specified module. For example, \c{eval(:(1+2))} will take the expression \c{:(1+2)} and return \c3.
\begin{jllisting}
for op in (:+, :*, :&, :|)
  eval(:(\$op(a,b,c) = \$op(\$op(a,b),c)))
end
\end{jllisting} %
\Eval is frequently used for meta-programming as part of code generation.
The above example uses \eval to generalize the basic binary operators to three
arguments, generating four new methods.

Julia's compilation model assumes that the set of callable methods for a given
invocation site is known at (JIT) compilation time. As mentioned previously,
the Julia JIT attempts to specialize invocation sites to devirtualize and inline
them, which then relies on knowing all possible methods that could be called.
A newly added method might be the new most specific applicable one for a call,
invaliding past optimizations.

Julia adds the world age mechanism to provide a consistent semantics for
dynamically generated code without needing to give the JIT the ability to back
out optimizations.The world-age mechanism limits the set of methods that can
be invoked from a given call site. World age fixes the set of method
definitions reachable from the currently executing method, isolating it from
dynamically generated ones. As a result, newly defined methods cannot be
invoked from previously compiled call sites due to the world age restriction,
and backing out/deoptimizing previous optimization decisions is no longer
needed. Moreover, it reduces the amount of global synchronization needed for a
multi-threaded program. 

Semantically, newly added methods (i.e. ones defined using \eval) only become
visible when execution returns to the top level, and the set of callable methods
for an execution is fixed when it leaves the top level. Compilation of methods
is triggered---only at the top level---when one of the following holds: (1) a
function is called with previously unobserved types of arguments, or (2) a
previously compiled function needs to be recompiled due to a change in its own
definition or one of its dependencies. Since the set of visible methods gets
fixed at a top-level call, and compilation only occurs from the top level, the
compiler may assume that the currently known set of methods is complete and can
optimize accordingly.

My goals for world age are twofold. First, I aim to formalize world age as it
is and show that its use as part of Julia's optimization strategy is correct
in the presence of \eval. Second, I will use it to justify the static type
system soundness claim in the presence of dynamically generated code.

\subsection{Multiple Dispatch.}

As mentioned previously Julia has \emph{multiple} dispatch, wherein it dispatches on every function argument. In contrast to a single dispatch language, where the runtime decides which method to call based on the first argument, called the receiver, Julia will dynamically pick the implementation to use based on the entire argument vector.

Earlier we explored how \jlinl{1+2} worked; Julia interprets the addition as a multimethod invocation to one of 190 different implementations:
\begin{jllisting}
# 190 methods for generic function "+":
[1] +(x::T, y::T) where T<:Union{Int128, Int16, Int32, Int64, Int8, UInt128, UInt16, UInt32, UInt64, UInt8} in Base
[2] +(c::Union{UInt16, UInt32, UInt8}, x::BigInt) in Base.GMP
[3] +(c::Union{Int16, Int32, Int8}, x::BigInt) in Base.GMP
[4] +(c::Union{UInt16, UInt32, UInt8}, x::BigFloat) in Base.MPFR
[5] +(c::Union{Int16, Int32, Int8}, x::BigFloat) in Base.MPFR
...
\end{jllisting}
Julia will pick which \jlinl{+} to use based on two criteria:
\begin{itemize}
    \item \emph{Applicability}: the method argument types must be supertypes of the
    dynamic argument typing. In this case, both \jlinl{1} and \jlinl{2} are \jlinl{Int64}s, so both the first and second arguments must be supertypes of \jlinl{Int64}. However, if no methods exist, then a ``method not found'' error is produced. For example, no method exists to add a string and a list, so \jlinl{"hello" + [1,2,3]} fails.
    \item \emph{Specificity}: whichever method is finally chosen must be the most specific method. Julia's definition of specificity is informal and practically motivated; a method can be more specific than another not only through subtyping, but through a number of additional ``useful'' rules described in~\cite{bezanson2018julia}. For example, \jlinl{Array{S} where S} is more specific than \jlinl{AbstractArray{String}} despite there being no subtyping relationship between the two types.
    
    If there are multiple most specific methods (methods that are more specific than any other alternative but are not more specific than one another), a ``method ambigous'' error is produced.If we add both \jlinl{+(::Int, ::Any) = 1} and \jlinl{+(::Any, ::Int) = 2} then try and call \jlinl{1+2} again, our two new definitions are more specific than any prior definition but neither is more specific than the other.
\end{itemize}

As implied by the use of dispatch to implement addition, Julia makes extensive use of multiple dispatch as part of its semantics. Almost all operations in Julia---beside new object creation, assignment, definitions, and control flow--are implemented using multimethod invocation. This extensive use of multimethods to define core functionality is what allows libraries to manipulate execution of code designed for ``normal'' Julia values, as the aforementioned Symbolics and ForwardDiff libraries do.

The way that libraries implement these extensions is by adding new definitions to existing multimethods. For example, if we load ForwardDiff and then look at the set of \jlinl{+} implementations, we now get
\begin{jllisting}
# 252 methods for generic function "+":
[...]
[109] +(x::ForwardDiff.Dual{Tx, V, N} where {V, N}, y::RoundingMode) where Tx in ForwardDiff
[110] +(x::ForwardDiff.Dual{Tx, V, N} where {V, N}, y::Rational) where Tx in ForwardDiff
[111] +(x::ForwardDiff.Dual{Tx, V, N} where {V, N}, y::Integer) where Tx in ForwardDiff
[112] +(x::ForwardDiff.Dual{Tx, V, N} where {V, N}, y::Irrational) where Tx in ForwardDiff 
[113] +(x::ForwardDiff.Dual{Tx, V, N} where {V, N}, y::AbstractFloat) where Tx in ForwardDiff
[114] +(x::ForwardDiff.Dual{Txy, V, N} where {V, N}, y::ForwardDiff.Dual{Txy, V, N} where {V, N}) where Txy in ForwardDiff
[115] +(x::ForwardDiff.Dual{Tx, V, N} where {V, N}, y::ForwardDiff.Dual{Ty, V, N} where {V, N}) where {Tx, Ty} in ForwardDiff
[116] +(x::ForwardDiff.Dual{Tx, V, N} where {V, N}, y::Real) where Tx in ForwardDiff
[...]
\end{jllisting}
There are now many more methods (we went from 190 to 252 by loading
ForwardDiff) and many of those came from ForwardDiff. Each of these new
implementations handles a case where some ForwardDiff type (in the above
example, ForwardDiff.Dual, the library's representation of a dual number) is
added to some existing value. It is possible to add new implementations that
solely manipulate types from other libraries or from the standard library, but
it is discouraged by the community (referred to as ``type piracy,'' as it is
seen as ``hijacking'' another libraries' type).

The ability to extend operations from other libraries, standard and otherwise,
with new types and behaviours allows the aforementioned composition of library
functionality. However, Julia has no formal mechanism for either checking that
these extensions are correct or that users are using values consistent with
what library developers expected.

As an example, many programs and libraries in Julia deal with arrays, and many
libraries want to define their own notion of array. For this purpose Julia
provides the \jlinl{AbstractArray} type, intended to be the supertype of all
array-like things in Julia. What array-like thing means, however, is somewhat
less defined: while \jlinl{AbstractArray} \emph{has} a list of methods that
implementers should provide, it exists solely in the Julia documentation.
Non-compliant implementations abound, even in the standard library, and thus a
developer who specified that an argument was a \jlinl{AbstractArray} could be
deeply surprised at any time.

The inability to statically know that an invocation will go through makes
Julia library programming difficult. One has to either program very
defensively (checking for the existence of required methods proactively and
dynamically) or accept that errors could occur almost randomly deep inside of
library code. Moreover, as in other dynamically typed languages, incorrect
typing of untested control flow paths can go unnoticed until a user stumbles
across it. 

I address this issue for Julia by providing both interface definitions,
allowing interfaces to be statically checked for compliance, and a static
gradual type system that can selectively check only some parts of a Julia
program.


\section{Thesis}

I argue that \emph{Julia can be gradually typed without modifiying the runtime}, based on three propositions:
\begin{enumerate}
\item \emph{A natural interpretation of gradual typing exists for Julia}; the concrete semantics aligns well with Julia's existing model of type membership.
\item \emph{We can abstract over Julia's subtyping mechanism}; the type system is ambivalent to type system modifications and does not need a comprehensive model of subtyping.
\item \emph{Performance is unaffected by typing}; no (new) runtime checks are required to ensure type soundness in the absence of metaprogramming.
\end{enumerate}

Thus, a gradual type system for Julia can be idiomatic and efficient.

==> Chapters/Chapter02.tex <==
%*****************************************
\chapter{Gradual Typing}\label{ch:examples}
%*****************************************

To begin gradually typing Julia we must first establish what it means to be
gradually typed. Logically, a gradual type system must accept some programs
and mark others as erroneous (or else it would not be a type system), but
exactly which programs are well-gradually-typed and which are not is not
agreed upon---a consequence of the varied enforcement strategies within each
system. 

Choice of enforcement strategy is one of the key decisions that the designer
of a gradual type system must make for it defines what it even means for a
value to be of a type; after all, if dynamic enforcment allows a string to be
typed as an integer, is that type all that meaningful? 

The instrumentality of enforcement to gradual typing begets several important
colloraries. First, from a social perspective, developers of a gradually-typed
language must be able to understand the details of the enforcement system to
write error-free code. Any gradual type system for an existing language must be
designed for it to be understandable to existing programmers. Second, and vitally
for this discussion, we can differentiate between gradual type systems solely
by what run-time errors they produce.

In order to discriminate between different gradual type systems and to provide
some intuition we propose a litmus test consisting of four programs written
in a common source language. The execution of each program varies depending
only on which gradual type system is being used for all are statically
well-typed and execute without error in a purely dynamic semantics. Errors
then arise based on  the choice of gradual typing semantics (and thus
enforcement strategy) that we apply in each case. We can then examine each
gradual type system through the lens of how it errors (or does not) for each
program.

\section{A Common Surface Language}

\begin{figure}[!t]\hrulefill \small\vspace{2mm}

{\bf Syntax:}\\[3mm]

\begin{tabular}{ll}
\begin{minipage}{6cm}\begin{tabular}{@{}l@{~}l@{}l@{}l@{}l@{}l@{}l@{}l}
\k~::=~ \Class \C {\fd[1]..}{\md[1]..} \qquad
\md~::=~\Mdef\m\x\t\t\e\qquad
\fd~::=~ \Fdef\f\t\qquad
\t~::=~ \any \B \C\\[3mm]
\K~::=~\k \K \B $\cdot$ \qquad
\Env~::=~\HT{\x}{\t} ~\Env \B $\cdot$ \qquad
\M~::=~\C <: \D ~\M \B $\cdot$ \\[3mm]
\e~::=~\x\B\this\B\FRead\f\B\FWrite\f\e\B\Call\e\m\e\B\New\C{\e[1]..}
\end{tabular}\end{minipage} 
\end{tabular}

\vspace{5mm}


{\bf Typing expressions:}\\[-6mm]

\begin{mathpar}
\Rule{STG-VAR}{~\\\\ 
  \HasType \Env\x\t
}{
  \EnvTypeS \Env\K\x\t
}

\Rule{STG-GET}{
  \HasType \Env\this\C \\\\  \Fdef\f\t \in \App\K\C
}{
  \EnvTypeS \Env\K{\FRead\f}\t
}    

\Rule{STG-SET}{
  \HasType \Env\this\C \quad \Fdef\f\t \in \App\K\C \\\\
  \EnvTypeS \Env\K\e\tp \quad  \ConvertE\K{s}\tp\t
}{
  \EnvTypeS \Env\K{\FWrite\f\e}\t
}    

\Rule[width=15em]{STG-CALL}{
  \EnvTypeS \Env\K\e\any \\\\ \EnvTypeS \Env\K\ep\t 
}{
  \EnvTypeS \Env\K{\Call\e\m\ep}{\any}
}    

\Rule[width=15em]{STG-CALL}{
  \EnvTypeS \Env\K\e\C \quad \EnvTypeS \Env\K\ep\t \\\\
  \Mtype \m{\t[1]}{\t[2]}\in \App\K\C  \quad
  \ConvertE\K{s}\t{\t[1]}
}{
  \EnvTypeS \Env\K{\Call\e\m\ep}{\t[2]}
}   

\Rule{STG-NEW}{
  \Ftype{\f[1]}{\t[1]}.. \in \App\K\C \\\\
  \EnvTypeS \Env\K{\e[1]}{\tp[1]}..\quad \ConvertE\K{s}{\tp[1]}{\t[1]}..
}{
  \EnvTypeS \Env\K{\New\C{\e[1]..}}\C
}
\end{mathpar}


{\bf Convertibility:}\\[-6mm]
  
\begin{mathpar}
\Rule{SUB}{ \SSub\cdot\K\t\tp}{ \ConvertE\K{s}\t\tp }
    
\Rule{TOA}{~ }{ \ConvertE\K{s}\t\any}
    
\Rule{ANYC}{~}{ \ConvertE\K{s}\any\t }
\end{mathpar}


{\bf Subtyping:}\\[-6mm]

\begin{mathpar}
\Rule{SAss}{  }{  \StrSub \M\K \any\any }

\Rule{SAss}{ \C \Sub \D \in \M }{  \StrSub \M\K \C\D }

\Rule{SRec}{
\M'=\C\Sub\D~\M\\\\\md\in\App\K\D\implies\mdp\in\App\K\C~.~\StrSub{\M'}\K\md\mdp
}{
 \StrSub \M\K \C \D 
}

\Rule{SMet}{
  \StrSub \M\K{\tp[1]}{\t[1]} \qquad \StrSub \M\K{\t[2]}{\tp[2]}
}{
 \StrSub\M\K{\Mdef\m\x{\t[1]}{\t[2]}\e}{\Mdef\m\x{\tp[1]}{\tp[2]}\ep}
}
\end{mathpar}

\hrulefill
\caption{Surface language syntax and type system (extract).}\label{slts}

\end{figure}

To provide a consistent presentation of each of the gradual type systems we
implement all of them on a single surface language. This surface language
is a gradually typed object calculus without inheritance, method overloading, or
explicit type cast operations. Figure~\ref{slts} provides its syntax as well
as an extract of its static semantics.

The key feature of our calculus is the presence of type \any, the dynamic
type. A variable of type \any can hold any value, invocations on type \any are
always statically well-typed, and expressionsof type \any can appear anywhere
within a typed program. Introducing \any converts our otherwise statically
typed surface language to a gradually typed language.

If we hypothesize the existence of a program without a \any type then that
program cannot get stuck; similarly, a program that only has \any types
may get stuck at any invocation. Gradual typing comes into play when static
and dynamic types interact such as an argument of type \any expected to be of
type \C or vice versa. The static type system permits such implicit coercions
through the convertability relation but may insert run-time checks to catch
potential type mismatches. The details of this cast insertion mechamism will be
described later; for now, we will rely on the reader's intuition.

Before presenting the litmus tests, some details about the type system of the
surface language may prove helpful. The subtyping relation is structural
with the Amber rule~\cite{cardelli1985amber} to enable recursion. \StrSub\M\K\C\D holds if class
\C has (at least) all the methods of class \D and the arguments and return
types are related by subtyping in the usual contra- and co-variant way; the
class table \K holds definitions of all classes, and \M is a helper for
recursion that records the subtype relations encountered so far. One noteworthy feature of subtyping is that the fields of objects
do not play a role in deciding if classes are subtypes. Following languages
like Smalltalk, fields are encapsulated and can only be accessed from within their
defining object. Syntactically, field reads and writes are limited to
the self-reference \this. 

The static type checking rules,   \EnvTypeS \Env\K\e\t where \Env is 
a type environment and \K is a class table,
 are standard with two exceptions: method invocation and convertibility. 
Method invocation is always allowed when the receiver \e is of 
type \any; therefore, \EM{\e.\m(\ep)} has type \any if the argument
can have type \any. Convertibility 
is used when statically typed and dynamically typed terms
interact. The convertibility relation, written $\ConvertE\K s\t\tp$, states
that type $\t$ is convertible to type $\tp$ in class table \K.  It
is used both for up-casting and for conversions of \any to non-\any types.
$\ConvertE\K s\t\tp$ holds when $\t\Sub\tp$, this allows up-casts. The
remaining two rules allow implicit conversion to and from the dynamic type.
To avoid collapsing the type hierarchy, convertibility is not transitive.
It is through convertibility that our surface language becomes gradual.



\subsection{Litmus}

Using four different programs, we can differentiate between five gradual
type systems. The litmus test is shown in \figref{litmus} and its
constituent programs are written in our surface language.  Each of these
programs consists of a class table and an expression whose evaluation in
the context of the class table determines if the litmus test succeeds or
fails.

The programs are designed to induce errors.  This is done by arranging for
values to cross typed/untyped boundaries in a way that will cause some type
systems to report an error but not others. At heart, these programs can 
be summarized by the
type boundaries that are crossed by an object. The
notation $\C ~\vert_{\,\t}$ denotes an object of class \C passing
through a boundary that expects it to be of type \t. For example,
if method \m expects an argument of type \t, a method call $\e.\m(\ep)$ would
induce the boundary $\ep ~\vert_{\,\t}$. 
In program {\bf L1}, we have:

\vspace{-5mm}
\[\A ~\vert_{\,\any} ~ \vert_{\,\I}\] 

\vspace{-2mm}\noindent
An instance of 
class \A is first implicitly converted to \any and then to \I; in this program
classes \A and \I are unrelated by subtyping. In {\bf L2}, the same sequence
of conversions is applied:

\vspace{-6mm}
\[\A~ \vert_{\,\any} ~ \vert_{\,\I}\] 

\vspace{-2mm}\noindent
This time \A and \I both have a
method \m, but the methods have incompatible argument types. In
{\bf L3} we start by converting a \C to \any and then to \E
and finally back to \any:

\vspace{-6mm}
\[\C~ \vert_{\,\any}~\vert_{\,\E}~\vert_{\,\any}\]

\vspace{-2mm}\noindent
The resulting value is then used to call  method \m with an argument of class \C.
This is correct as method \m in \C does expect an
argument of that type. If the object was an instance of \E, instead, the call
would not be legal because \E's method \m expects a class \D as argument.

Example {\bf L4} is more complex as it relies on one value to apply a type constraint
on another. The first value begins life as a \C, is cast to \any, then is aliased. On
one leg it is cast to a \D and is promptly forgotten about. On the other it is cast
back to a \C and then to \any. We will refer to the result of this second branch as \EMxt v.

\vspace{-6mm}
\begin{align*}
\C~ \vert_{\,\any}~&\vert_{\,\D} \\
    &\vert_{\,\C}~\vert_{\,\any} \rightarrow \EMxt v
\end{align*}

\vspace{-2mm}\noindent
The second value in L4, too, begins life as a \C. It is passed to the
\EMxt{f} of \EMxt v which may then enforce a type (denoted ?) upon it.

\vspace{-6mm}
\begin{align*}
\C~\vert_{\,?}
\end{align*}

\vspace{-2mm}\noindent

\begin{figure}[!b] 
\begin{minipage}{0.5\textwidth}
\begin{lstlisting}
class A {
	m(x:A):A {this} }



class I {
	n(x:I):I {this} }


class T {
	s(x:I):T {this}
	t(x:*):* {this.s(x)} }
\end{lstlisting} \vspace{-2em}
\begin{lstlisting}
new T().t(new A())
\end{lstlisting}
\end{minipage}
\begin{minipage}{0.5\textwidth}
\begin{lstlisting}
class A {
	m(x:A):A {this} }

class Q {
	n(x:Q):Q {this} }

class I {
	m(x:Q):I {this} }

class T {
	s(x:I):T {this}
	t(x:*):* {this.s(x)} }
\end{lstlisting}\vspace{-2em}
\begin{lstlisting}
new T().t(new A())
\end{lstlisting}
\end{minipage}
\\
\begin{minipage}{0.5\textwidth}
\begin{lstlisting}
class C {
	a(x:C):C {x} }

class D {
	b(x:D):D {x} }

class E {
	a(x:D):D {x} }


class F {
	m(x:E):E {x}
	n(x:*):* {this.m(x)} }
\end{lstlisting}\vspace{-2em}
\begin{lstlisting}
new F().n(new C())
	   .a(new C())
\end{lstlisting}
\end{minipage}
\begin{minipage}{0.5\textwidth}
\begin{lstlisting}
class C { f(x:*):* {x} }
class D { f(x:I):I {x} }
class I { dif(x:*):* {x}}


class T {
	f1:C f2:D
	first(x:*):* {this.f1} }


class E {
	alias(x:*):* {
		new T(x, x).first(x) } }
\end{lstlisting}\vspace{-2em}
\begin{lstlisting}
new E().alias(new C())
       .f(new C())
\end{lstlisting}
\end{minipage}

  \caption{Litmus test. Each program consists of a class table (top) and
    an expression (bottom). Top left table indicates successful
    executions.}\label{litmus}
\end{figure}

\noindent We will use this litmus test to differentiate between four different
gradual type systems:

\vspace{2mm}\noindent
{\bf Optional.~} An optional gradual type system simply erases all of the
type annotations at run-time; all four programs run to completion without
error.

\vspace{2mm}\noindent {\bf Concrete.~} The concrete approach ensures that a
variable of some class \C always refers to an object of that class or of a
subtype of it.  To ensure this is the case, all implicit conversions imply a
run-time subtype check.  This causes three of four programs to fail. {\bf L1}
and {\bf L2} fail on a subtype test \StrSub{}\K\A\I.  {\bf L3} fails on the
subtype test \StrSub{}\K\C\E. {\bf L4} runs successfully; the value of the 
placeholder ? type is \any under the concrete semantics as \C's implementation
is used.

\vspace{2mm}\noindent {\bf Behavioral.~} The behavioral approach allows
conversion from \any to \C if the value is compatible to \C and if,
after that, it behaves as if it was an instance of \C.  The former is
checked by a shallow cast that only looks at method names, and the
latter by a wrapper that monitors further interactions.  {\bf L1} fails at
because \A does not have the method \xt n expected by \I. {\bf L2}, however,
executes without error because \A has the method \m expected by \I. {\bf L3} fails, since the instance of \C has acquired
a wrapper for \E.  When method \a is called with a \C, the wrapper notices
that \E's method \a expects a \D and that \C and \D are not compatible. Finally,
{\bf L4} succeeds as \EMxt v is never wrapped and thus the placeholder is again
\any, taken from \C.

\vspace{2mm}\noindent {\bf Transient.~} The transient approach is weaker
than behavioral. It retains the shallow structural checks at casts of the
behavioral approach, but does not wrap values. Transient fails {\bf L1}, for
the same reason as the other two type systems, and passes {\bf L2}, for the
same reason as behavioral.  {\bf L3} succeeds because transient forgets that
the \C object was cast to \E. {\bf L4} also succeeds and \EMxt v is similarly
only ever cast to \any.

\vspace{2mm}\noindent {\bf Monotonic.~} The monotonic approach sits in between
transient and behavioural; it ensures that all references to heap values are
well typed by continously specializing the heap. {\bf L1} fails and {\bf L2}
succeed for the same reasons as when running under the behavioural semantics.
{\bf L3} fails as the monotonic semantics specializes method definitions to
ensure their behavioural type-correctnes with respect to all references.
Finally, {\bf L4} fails as \f on \EMxt v has been specalized in the heap to
enforce the type signatures applied by the cast to \D on the opposing branch.
As a result, the program fails on the cast from \C to the instantiation of ?
(in this case \EMxt I) as the two types are structurally incompatible.


\subsection{Discussion}

These tests capture the behavior of implementations. The three have been
expressed in TypeScript (optional), StrongScript (concrete), Typed Racket
(behavioral) and Reticulated Python (transient), with the same
errors.\footnote{\small
  \url{github.com/BenChung/GradualComparisonArtifact/examples}}
What the litmus tests show is that a precise understanding of the semantics
of gradually typed languages, and their run-time enforcement machinery, is
crucial for developers to know if a program is ``correct.''  Here, all
errors are false positives, since none of these programs performs an invalid
operation. This underlines the fact that in gradually typed language, type
specifications can lead to run-time errors just as faulty code can. Thus,
type annotations must be audited and tested just like code.

These approaches induce usability trade-offs. One way to contextualize this
is with the gradual guarantee of Siek et
al~\cite{GradualGuarantee}. Informally, it states that if there exists a
static type assignment to an untyped program that allows the program to run
to completion, any partial assignment of those types will do too. The
optional approach trivially fulfills this guarantee.  Transient likewise
satisfies the gradual guarantee~\cite{Vitousek2017}, as it only checks
top-level structure of values at type boundaries. Unlike optional, transient
does ensure that typed calls succeed; however, a call may produce a dynamic
error if the receiver is of the wrong type (even in a typed context), or the
return is an ill-typed value.  The behavioral approach also fulfills the
guarantee, as it only checks arguments and return types when wrappers are
invoked. However, typed function calls can fail if they call an untyped
function that returns the wrong value. Finally, the concrete approach
ensures that every typed call is successful. However, this comes at the
expense of the gradual guarantee --- partially typed classes are not
compatible with more-or-less typed ones.  The guarantee
is incompatible with subtyping. Suppose a program were to rely on the
judgment $\{m(\C):\D\} <: \{m(\C):\D\}$.  Relaxing the argument type to a
dynamic type, $\{m(\any):\D\} <: \{m(\C):\D\}$, violates subtyping.  To
overcome this, Reticulated Python augments subtyping with the aforementioned
consistency relation. This increases the number of programs accepted by the
static type system. However, it is not used by the run-time semantics and
is fundamentally incompatible with the concrete approach (because any use of
consistent subtyping will fail).  We omit consistent subtyping.

As an alternative consider the approaches taken by Thorn or
StrongScript. They have three kinds of types: \any (dynamic), \C (concrete),
and \xt{like} \C (optional), combining the concrete and optional approach
into the same language. This design allows for a different kind of
migration; once a program is fully annotated with optional types, they all
can be converted to concrete types without introducing any run-time
errors~\cite{ecoop15}.  We do not model this combination directly, as the
underlying details are no different from the concrete approach.

The motivation for making fields private is to simplify the system. With
private fields, errors are limited to method invocation. Field accesses can
be trivially checked; as they are always accessing \this. Moreover, interposing on
method invocation can easily be achieved by wrappers, whereas interposing
on field access would require modifying the code of clients. This would make
the formal development more cumbersome without adding insight.


\section{KafKa: A Core Calculus}\label{kafkacore}

\noindent Even without gradual typing, comparing languages is difficult.
Small differences in syntax and features can make even the most similar
languages appear different. As a result, the nuances of gradual type systems
are often hidden amongst irrelevant details.  To enable direct comparison,
we propose to translate gradually typed languages down to a common calculus
designed to highlight the distinctions between designs.  The target for this
translation is our core language, \kafka. \kafka is a statically typed
language similar to the surface language but with several features added to
enable its use as a common target language.

These additions make an explicit distinction between static and dynamic
operations and replace implicit conversions with explicit casts.  \kafka's
first additions consist of three casts which are used at boundaries between
typed and untyped code: 
\begin{itemize}
	\item \SubCast\t\e, \emph{concrete} casting, which ensures that expression \e evaluates to a subtype of \t.
	\item \BehCast\t\e, \emph{behavioural} casting, which adds a wrapper around the value of \e that monitors \e to ensure that it behaves as if it was of type \t.
	\item \MonCast\t\e, \emph{monotonic} casting, which recursively specializes the heap to comply with type \t.
\end{itemize}
Additionally, a syntactic distinction is made between static method
invocation, written \KCall\e\m\ep\t\tp, dynamic method invocation,
\DynCall\e\m\ep.  Static invocations does not get stuck, whereas
dynamic invocations can. This makes explicit which function calls can fail.

\kafka was designed to align with common statically-typed class-based
object-oriented compilation targets like .NET or the JVM. It maps to the
intermediate language supported by these platforms. \kafka also requires the
ability to generate new classes at run-time, a feature supported by these
environments but typically not present in class-based calculi.

\renewcommand{\S}{\EM{\Sigma}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[!h]\small\noindent\hrulefill

\vspace{4mm}
{\bf Syntax:}
\vspace{2mm}

\begin{tabular}{@{}ll}\hspace{5mm}\begin{minipage}{7.2cm}\begin{tabular}{@{}l@{~}l@{}l@{}l@{}l@{}l@{}l@{}l}
\e\hspace{.1cm} ::=  \hspace{.2cm} 
 & \x       &\B \this       &\B \that  & \B   \\
 & \FRead\f &\B \FWrite\f\e &\B \New\C{\e[1]..} &\B\\
 & \KCall\e\m\e\t\t   &\B \DynCall\e\m\e &\B\\
 & \SubCast\t\e  &\B \BehCast\t\e & \B \\
 &  \a  &\B \FReadR\a\f &\B \FWriteR\a\f\e 
\end{tabular}\end{minipage}&
\begin{minipage}{2.4cm}\begin{tabular}{l@{~}l@{}l@{}l}
  \k &::= ~ \Class \C {\fd[1]..}{\md[1]..} \\
 \md &::= ~ \Mdef\m\x\t\t\e \\ 
 \fd &::= ~ \Fdef\f\t \\ 
  \t &::= ~ \any  \B   \C  \\ 
  \K &::= ~ \k \K \B $\cdot$ \\
  \S &::= ~ \HT\a\t $\Sigma$ \B $\cdot$ \\
\end{tabular}\end{minipage}\end{tabular}

\vspace{6mm}
{\bf Static semantics:}
\vspace{-2mm}


\begin{mathpar}
\Rule{W6}{
  \EnvType \Env\S\K\e\C \\
  \Mtype\m\t\tp \in \App\K\C  \\
  \EnvType \Env\S\K\ep\t
}{
  \EnvType \Env\S\K{\KCall\e\m\ep\t\tp}\tp
}    

\Rule{W7}{
  \EnvType \Env\S\K\e\any \\
  \EnvType \Env\S\K\ep\any
}{
  \EnvType \Env\S\K{\DynCall\e\m\ep}\any
}    

\\

\Rule{W9}{
  \EnvType \Env\S\K\e\tp
}{
  \EnvType \Env\S\K{\SubCast\t\e}\t
}

\Rule{WB}{
  \EnvType \Env\S\K\e\tp
}{
  \EnvType \Env\S\K{\BehCast\t\e}\t
}

\Rule{W9}{
  \S(\a) = \C
}{
  \EnvType \Env\S\K\a\C
}

\Rule{W10}{
 }{
   \EnvType \Env\S\K\a\any
}
\end{mathpar}


\vspace{4mm}
{\bf Execution contexts:}
\vspace{-2mm}

\[
\begin{tabular}{llllllllllllllllll}
\EE &::=& ~ \FWriteR\a\f\EE   &\B  
        \KCall\EE\m\e\t\t  &\B
        \KCall\a\m{\EE}\t\t &\B
        \DynCall\EE\m\e   &\B\\
&       & \DynCall\a\m\EE   &\B
       \SubCast\t\EE  &\B
      \BehCast\t\EE  &\B
       \New\C{\a[1]..\,\EE\,\e[1]..} &\B 
      \EM{\square}
\end{tabular}
\]

\vspace{4mm}
{\bf Dynamic semantics:}
\vspace{2mm}

\hspace{7mm}\begin{minipage}{\textwidth}

\begin{tabbing}
\K\HS \New\C{\a[1]..} \HS\=\s~\HS\=\Red\HS\=\K\HS\=\ap\HS~\= \sp\HS \= \WHERE\HS\= \fresh\ap \HS\HS\HS\HS\HS\HS\HS\=  \sp = {\Map\s{\Bind\ap{\obj\C{\a[1]..}}}}
\\
\K\HS \FReadR\a{\f[i]} \> \s           \>\Red\>     \K \>$\a[i]$ \> \s  \> \WHERE \>\App\s\a=\obj\C{\a[1],\ldots\a[i],\a[n]\ldots}
\\
\K\HS {\FWriteR\a{\f[i]}\ap} \> \s     \>\Red\>     \K \> \ap \> \sp \>  \WHERE \>\App\s\a=\obj\C{\a[1],\ldots\a[i],\a[n]\ldots} \HS  
\\ \> \> \> \> \> \> \> \sp = \Map\s{\Bind\a{\obj\C{\a[1],\ldots\ap,\a[n]\ldots}}}
\\
\K\HS{\KCall\a\m\ap\t\tp} \> \s      \>\Red\>     \K \>  \ep \> \s \> \WHERE\> \ep = {[\a/\this~{\ap/\x}]\e} \HS \\ \> \> \> \> \> \> \> \Mdef\m\x{\t_{1}}{\t_{2}}\e\In \App\K\C  \\ \> \> \> \> \> \> \>  \App\s\a=\obj\C{\a[1]..} \> \StrSub {\emptyset}\K\t {\t_{1}} \\ 
\> \> \> \> \> \> \> \StrSub {\emptyset}\K{\t_{2}} \tp
\\
 \K\HS {\DynCall\a\m\ap}\> \s        \>\Red\>    \K \> \ep \> \s \>  \WHERE\> \ep = {[\a/\this~{\ap/\x}]\e}\HS \\ \> \> \> \> \> \> \> \Mdef\m\x\any\any\e \In \App\K\C \\ \> \> \> \> \> \> \> \App\s\a=\obj\C{\a[1]..} 
\\
 \K\HS {\SubCast \any\a} \> \s       \>\Red\>   \K \> \a \> \s
\\
 \K\HS {\SubCast \D\a} \> \s        \>\Red\>    \K \> \a \> \s \>  \WHERE\> \StrSub {\emptyset}\K\C \D \>\App\s\a=\obj\C{\a[1]..} 
\\
 \K\HS {\BehCast \t\a} \> \s         \>\Red\>   \Kp \> \ap \> \sp \> \WHERE\> \behcast \a\t\s\K \Kp\ap\sp    
\\
\K \HS \EM{\EE[\e]} \> \s            \>\Red\>   \Kp \> \EM{\EE[\ep]} \> \sp \> \WHERE \> \K~\e~\s \Red~\Kp~\ep~\sp
\end{tabbing}
\end{minipage}

\medskip
\hrulefill
\caption{\kafka dynamic semantics and static semantics
  (extract).}\label{fig:kafka}
\end{figure}


\subsection{Syntax and Semantics}

We had two requirements when designing \kafka: first, to be expressive enough to
capture the dynamic semantics implied by each gradual type system; second,
to have a type system that can express when code is known to be error
free. \kafka's syntax and semantics, loosely inspired by Featherweight
Java~\cite{FJ}, are shown in \figref{fig:kafka}.  At the top level, classes
are notated as \Class\C{\fd[1]..}{\md[1]..}; methods, ranged over by \md,
are denoted as \Mdef\m\x\t\t\e; and fields \Fdef\f\t. Expressions consist
of:

\vspace{-3mm}

\begin{itemize}
\item variables, \x;
\item the self-reference \this; and wrapper target, \that;
\item field accesses, \FRead\f, and field writes, \FWrite\f\e;
\item object creation, \New\C{\e[1]..};
\item static and dynamic method invocations;
\item subtype and behavioral casts;
\item and heap addresses.
\end{itemize}

\noindent
The static semantics holds only a few surprises; key typing rules appear in
\figref{fig:kafka}. The subtyping relation is inherited from the surface
language.  The program typing relation (not shown here), \WFp\e\K, indicates
that expression \e is well-formed with respect to class table \K. The
expression typing judgment $\EnvType \Env\S\K\e\t$, indicates that against
\Env with heap typing \S and class table \K, \e has type \t.  Unlike the
surface language, \kafka does not rely on a convertibility relation from
\any to \C and back; instead, explicit casts are required.

Evaluation is mostly standard with an evaluation context consisting of a
class table \K, the expression being evaluated \e, and a heap \s mapping
from addresses \a to objects, denoted $\C\{\a\ldots\}$. Due to the need for
dynamic code generation, the class table is part of the state.

\subsubsection{Method Invocation}

\kafka has two invocation forms, the dynamic \DynCall\e\m\ep and the static
\KCall\e\m\ep\t\tp, both denoting a call to method \m with argument \ep.
There are several design issues worth discussing.  First, as our calculus is
a translation target, it is acceptable to require some explicit preparation
for objects to be used in a dynamic context.  A dynamic call is only
successful if the receiver has a method of the expected name and with
argument and return types of \any. This is a design choice of \kafka, even
dynamic invocation has to be well-typed (even if this typing is
trivial).  Secondly, it is possible for a static invocation to call an untyped
method (of type \any to \any).
Consider the following
class definition

\newcommand{\Int}{\xt{Int}}

\begin{tabbing}
\small\hspace{2cm}\class \C \=\{\\
 \>\HS\HS\Mdef\m\x\Int\Int{\HS\x+2\HS}\\
 \>\HS\HS\=\m(\x:~\any)~:~\any\{~\SubCast\any{\KCall\this\m{\SubCast\Int\x}\Int\Int}~\}\\
     \> \}
\end{tabbing}

\noindent
assume that class table \K holds a definition for \Int, and that we have
integer constants and addition.
The class demonstrates several features of \kafka. Its class
well-formedness rules (not shown here) allow a limited form of method
overloading. A class may have at most two occurrences of any method \m: one 
``untyped'' with \any as argument and return type; and one,
which we call ``typed'', where either its argument or return type differ from \any.
The static type system enforces a single means of invoking a typed method
\m:

\vspace{-6mm}\[\KCall{\New\C{}}\m{2}\Int\Int\] \vspace{-5mm}

\noindent
Here, the receiver is obviously of type \C and the argument is \Int; thus, the
call is statically well-typed. The expression will therefore 
evaluate the body of \m.  For an untyped method, there are two invocation
modes:

\vspace{-6mm}\[\DynCall{\New\C{}}\m{2}\]\vspace{-5mm}

\noindent The call executes correctly here, as \C has an untyped \m. However,
in the general case, there is no guarantee that the receiver of an untyped
invocation has the requested method; and therefore, a dynamic invocation can
get stuck. The receiver of a dynamic invocation has type \any.  When the
receiver type is known to be some \C and that class has the requested method,
then the static invocation can be used:

\vspace{-6mm}\[\KCall{\New\C{}}\m{2}\any\any\]\vspace{-5mm}

\noindent The invocation will succeed. All nuances of invocation
will come in handy when translating the surface language to \kafka.

\subsubsection{Run-time Casts}

\kafka has two cast operations: the structural subtype cast $\SubCast\t\e$ and the
behavioral cast $\BehCast\t\e$, both indicating the desire for the result
of evaluating \e to be of type \t.  Where the casts differ is what is meant by
``has type \t''.  The subtype cast checks that the result of evaluating \e
is an object whose class is compatible with \t. If \t is a class, then it
will check for a subtyping relation; otherwise, if \EM{\t=\any}, the cast 
will succeeds. As every value in the heap is
tagged by its type constructor, it is always possible to perform this check. 
The behavioral cast is more complex; we will
describe it in the remainder of this section.

The objective of the behavioral cast is to ensure that the wrapped object
behaves as the target type dictates. When given the address \a of some
object, this cast creates a wrapper object, say \ap, that enforces the 
invariant that \a \emph{behaves} as a
value of type \t.  Function \behcastE\a\t\s\K \Kp\ap\sp specifies its
semantics, shown in \figref{behavetext}.  There are two cases to consider:
either the target type is a class \Cp, or it is \any.

\begin{figure}[!h]\hrulefill\small

\vspace{4mm}
{\bf Behavioral cast:}
\vspace{4mm}
\behcastE\a\t\s\K \Kp\ap\sp\\[2mm]
\begin{tabular}{ll|ll}
\a & Reference to wrap & \ap & Wrapped reference \\
\t & Target type to enforce & \Kp & Class table with wrapper\\ 
\s & Original heap & \sp & New heap \\
\K & Original class table &
\end{tabular}

\vspace{4mm}

\begin{equation*}
\behcastE\a\Cp\s\K \Kp\ap\sp \HS\WHERE\HS \begin{cases}
 \HS\App\s\a = \obj\C{\a[1]..} \HS\HS    \fresh{\D,\ap} \HS\HS
  \sp = \Map \s{\Bind\ap{\obj\D{\a}}} \\\HS
  \md[1].. \In\App\K\C \HS\HS \names{\mdp[1]..} \subseteq \names{\md[1]..} \\\HS
  \mdp[1].. \In \App\K\Cp \HS\HS \cload{\md[1]..} \HS \cload{\mdp[1]..} \\\HS
  \Kp = \K ~\wrap\C{\md[1]..}{\mdp[1]..}\D 
  \end{cases}
\end{equation*}

~\\[-8mm]

\begin{equation*}
  \behcastE\a\any\s\K \Kp\ap\sp  \HS\HS\WHERE\HS\HS\begin{cases}\HS
  \App\s\a = \obj\C{\a[1]..} \HS\HS \md[1].. \In \App\K\C \HS\HS
  \fresh{\D,\ap} \\\HS \cload{\md[1]..} \HS\HS
  \Kp = \K ~ \wrapAny\C{\md[1]..}\D \\\HS
  \sp = \Map \s{\Bind\ap{\obj\D{\a}}} 
\end{cases}\end{equation*}

\vspace{4mm}

\hspace{8mm}\begin{minipage}{12cm}\begin{tabbing}\small
  \wrap\C{\md[1]..}{\mdp[1]..}\D = \src{\Class\D{\Fdef\that\C}{\mdpp[1]..}}\\
  \HS\HS\WHERE\HS\= \Mdef\m\x{\t[1]}{\t[2]}\e\In\md[1].. \\
                 \> \mdpp[1] =\= \src{\Mdef\m\x{\tp[1]}{\tp[2]}{~\BehCast{\tp[2]}{\KCall{\FRead\that}\m{\bscast{\t[1]}\x}{\t[1]}{\t[2]}}}} .. \\
\> \> \HS\HS \= \textbf{if} \HS \Mdef\m\x{\tp[1]}{\tp[2]}\ep\In\mdp[1].. \\
\\[-3mm]
\> \>  \src{\Mdef\m\x{\t[1]}{\t[2]}{~\KCall{\FRead\that}\m{\x}{\t[1]}{\t[2]}}} .. \\ \> \> \HS\HS \textbf{otherwise}
\\[2mm]
  \wrapAny{\C}{\md[1]..}{\D} = \src{\Class \D{ \Fdef\that\C}{ \mdp[1]..}}\\
\HS\HS\WHERE\HS\=\mdp[1] = \src{ \Mdef\m\x{\any}{\any}{~\BehCast\any{ \KCall{\FRead\that} \m {\bscast{\t}\x}{\t}{\tp}} } }   ..
    \HS\HS\HS\HS \\ \> \> \HS\HS \= \textbf{if} \HS \Mdef\m\x{\t}{\tp}\e\In\md[1].. \\
\end{tabbing}\end{minipage}

\vspace{-2mm}

\hrulefill
\caption{Behavioral cast semantics.}\label{behavetext}
\end{figure}

\newcommand{\W}{\xt{W}\xspace}

If the target type is \Cp, then \behcastS\a\Cp\s\K will return an updated
class table \Kp, a reference to the wrapped object \ap, and an updated heap
\sp. As long as \a has every method name specified by \Cp, the cast itself
will succeed. If \a is missing a method, it is impossible for \a to
implement \Cp correctly, and early failure is indicated. Otherwise, the
metafunction continues to generate a type wrapper. Class generation itself
is delegated to the \W metafunction.  A \W invocation,
\EM{\W(\C,\md_1..,\mdp_1.., \D)}, takes a class \C, a fresh name \D, and two
method lists $\md_1..$ and $\mdp_1$, respectively the method of \C and the
methods of the type to enforce.  The class generated by \W will have adapter
methods for each method \m occurring in both $\md_1..$ and $\mdp_1..$. Type
mismatches between the wrapped object and the wrapping type are resolved
with more behavioral casts. For methods that do not need to be adapted
(methods only in $\md_1..$), a simple pass-through method is generated. This
method simply calls the wrapped object; itself referred to by the
distinguished variable \that.

If the target type is \any, the wrapper class is simpler. It only needs to
check that method arguments match the types expected by the wrapped
object. This is done by another behavioral cast. Return values are cast to
\any.

For example, consider the following program which has two classes \C and \D.
Even though \C and \D both have method \a, they are not subtypes because the
arguments to their \m implementations are not related.

\begin{tabbing}\small
\hspace{1cm}
\Call{(\BehCast\C{(\BehCast\D{\New\C{}})})}{\xt{b}}{2} \HS\HS\HS\WHERE\HS
  \K\HS =\HS \= \class\= \C \{\\
       \> \HS \Mdef\m\x\any\any{\HS\x\HS}\\
       \> \HS \Mdef\n\x\any\any{\HS\x\HS}\\
       \> \}  \\
       \>\class \D \{\HS \Mdef\m\x\Int\Int{\HS\x\HS}\HS \}
\end{tabbing}

\noindent
The program starts with a \C, casts it to \D, and then back to \C. The
reason we generate pass-through methods (the wrapper that enforces type \D
has a method \n) is that without them, the method \n would be ``lost''. 
Without the pass-through method, it would be impossible to cast back to
\C, as the wrapper would only have an implementation for \m. Wrappers
with this semantics are referred to as opaque, as it is not possible
to see methods of the underlying object though them. In contrast,
\kafka uses transparent wrappers.
To illustrate what this looks like, the following class \xt E is generated
by the cast from \C to \D:

\begin{tabbing}\small
\HS\HS\=\class\= \xt E \{\\
\>\> \HS \Fdef\that\C \\
\>\> \HS \Mdef\m\x\Int\Int{\HS\BehCast\Int{\KCall\that\m{\BehCast\any\x}\any\any\HS}} \\ 
\>\> \HS \Mdef\n\x\any\any{\HS \KCall\that\n{\x}\any\any\HS} \\ 
\>\}
\end{tabbing}

\noindent
By keeping \n present, it is possible to return an instance of
\E to \C again. If we were to remove \n, then \xt E would no longer
be convertible back to \C again.    

\subsection{Type soundness}

The \kafka type soundness theorem ensures that a well-formed program can
only get stuck at a dynamic invocation, a subtype cast, or a behavioral
cast, and only there when justified.

\begin{theorem}[\kafka type soundness]

\noindent For every well-formed state $\WFq{\K~\e~\s}$ and well-typed
expression $\EnvType\emptyset\S\K\e\t$, where heap typing \S is obtained by
mapping the class of each object to the corresponding address, one of the
following holds:

\newcommand{\Sp}{\EM{\S'}\xspace}

\begin{itemize}
\item There exists some reference \a such that $\e = \a$.
\item $\K~\e~\s\Red\Kp~\ep~\sp$, where $\WFq{\Kp~\ep~\sp}$,
  \EnvType\emptyset\Sp\Kp\ep\t, \sp has all of the values of \s, \Sp has all of the
  types of \sp, and \Kp has all of the classes of \K.
\item $\e=E[\DynCall\a\m\ap]$ and \a refers to an object without a method \m.
\item $\e=E[\SubCast\C\a]$, and \a refers to an object whose class is not
  a subtype of \C.
\item $\e=E[\BehCast\C\a]$, and \C contains a method that \a does not.
\end{itemize}
\end{theorem}

\noindent
The proof is mostly straightforward, with one unusual case, centered around
the \xt{bcast} metafunction. When the \xt{bcast} metafunction is used to
generate a wrapper class, which is then instantiated, producing a new class
table and heap, we must then show that the new class table is well formed,
that the new heap is also well formed, and that the new wrapper is a subtype
of the given type \C.  Proving these properties is relatively easy.  Class
table well-formedness follows by construction of the wrapper class and by
well-formedness of the old class table. Heap well-formedness follows by
well-formedness of the class table, construction of the new heap, and
well-formedness of the old heap.  Proving that the type of the wrapper is a
subtype of the required type proceeds by structural induction over the
required type.  The proof of soundness has been formalized in Coq and is
available in the supplementary material. The proof relies on two axioms
dealing with recursive structural subtyping. We did not prove these as
they have been shown in prior work~\cite{JonesStructural}.

\subsection{Discussion}

The design of \kafka's two invocation forms bears discussion. In some
previous works, dynamic invocation has been implemented by a combination of
a cast and a statically typed call.  In our case, following this approach
would require creating a type for each invocation (as was done
in~\cite{popl10}). Instead, providing a dynamic invocation form seemed more
natural.  The use of explicitly typed invocation is a result of our desire
to be able to rule out more errors statically. Whenever a translation can
generate a static invocation, the soundness result ensure that the call will
succeed. But, some methods need to be called from both a typed and untyped
context, to achieve this we generate two versions of the method and leverage
the difference between typed and untyped calls to express invovations
occuring in each context.

One of our requirements for \kafka was that it support transparent wrappers
as these are needed for the behavioral approach. The combination of
structural subtyping and dynamic class generation allows to generate
subtypes on the fly. These subtypes have all the methods of the target type
plus some new ones. The choice of having fields be private means that the
wrappers do not have to special case field access. If fields were accessible
from outside the object, some more complex rewritting would have to be
used.

\kafka was intended to match the intermediate languages of commercial VMs.
To validate this, we implemented a compiler from \kafka to
C\#.\footnote{\small\url{github.com/BenChung/GradualComparisonArtifact/netImpl}}
The only challenge was due to subtyping. \kafka uses structural typing,
while C\# is nominal, and \kafka allows methods in subtypes to be
contra-variant in argument and co-variant in return type, while C\# requires
invariance.  Implementing structural subtyping on top of a nominally typed
language is tricky. Structural types create implicit subtyping
relationships, which the nominal type system expects to be explicit.  Prior
work used reflection and complex run-time code
generation~\cite{StructuralTypesOnJVM}, but this is needlessly complex for a
proof of concept.  Instead, we reify the implicit relationships introduced
by structural subtyping into explicit nominal relationships by generating
interfaces. Given two classes \C and \D, where $\K\vdash \C \Sub \D$ holds,
we generate two interfaces \xt{CI} and \xt{DI}, where \xt{CI} is declared to
extend \xt{DI}. As a result, if two types are subtypes, their corresponding
C\# interfaces will be as well.  The next problem is that \kafka allows
subtype methods to be contra-variant in argument and co-variant in return
types.  As a result, a single method in \xt{CI} may not be sufficient to
implement \xt{DI}.  We solve this by having every class's C\# equivalent
implement every interface explicitly, with each explicit implementation
delegating to the real, most general, implementation.  Despite these issues,
we were able to accurately translate \kafka types. We translate static and
dynamic invocations into corresponding C\# invocations since C\# also has a
dynamic type. The underlying run time can then use the translated \kafka
types to perform method dispatch, while inserting dynamic checks wherever
the \kafka code calls for an untyped invocation. This prototype shows that
\kafka primitives are close to those of intermediate languages. As a result,
the translation of gradual type systems to \kafka provides insight as to how
they might be implemented.



\section{Translating Gradual Type Systems}


\noindent Equipped with the source and target languages, we can describe
the gradual-to-statically typed translation from source to \kafka.
Each semantics is translated through a function mapping well-typed
surface programs into well-typed \kafka terms. The translation
explicitly determines which type casts need to be inserted and the
invocation forms to use. A type-driven translation will insert casts
where the surface language used consistency.

\subsection{Class Translation}

The translations for surface level classes are shown in
\figref{fig:traclass}. Each class in the surface language translates to a
homonymous \kafka class, retaining type names through translation.
The grey background denotes code generated in the translation.
The notation \EM{\e;\ep} denotes sequencing. 

\begin{figure}[!b]  {\small  \hrulefill\\
\begin{tabular}{llc@{\hspace{.25cm}}l}     \\[-2mm]

{\bf Optional:} \\[1mm]

\HS\TR[\OTS]{\Class\C{\fd[1]..}{\md[1].. }}
   & = \src{\Class\C{\fdp[1]..}{\mdp[1]..}}\\     
   & \WHERE\HS\HS\HS \fdp[1] = \src{\Ftype\f\any}..\HS\HS \fd[1] = \Ftype\f\t..\\
   & \HS\HS\HS\HS\HS\HS\HS\HS\HS  \mdp[1] = \src{\Mdef\m\x\any\any\ep}..\\   
   & \HS\HS\HS\HS\HS\HS\HS\HS\HS \md[1] = \Mdef\m\x{\t[1]}{\t[2]}\e \HS\HS
                                 \ep=\;\TR[\OTS]{\e}\\   
        
{\bf Transient:} \\[1mm]   
\HS\TR[\TTS]{\Class\C{\fd[1]..}{\md[1]..}}
    & = \src{\Class\C{\fdp[1]..}{\mdp[1]..}}\\   
    & \WHERE \HS\HS\HS \fdp[1] = \src{\Ftype\f\any} .. \HS    
    \fd[1] = \Ftype\f\t ..\HS\HS \\   
    & \HS\HS\HS\HS\HS\HS\HS\HS\HS \mdp[1] = \src{\Mdef\m\x\any\any{\SubCast\t\x ~; ~\ep[1]}} .. \\    
    & \HS\HS\HS\HS\HS\HS\HS\HS\HS \md[1] = \Mdef\m\x\t\tp\e .. 
   \HS \HS \ep[1] = \TAG[\TTS]\e{\x:\t\,\this:\C}\any~ .. \\        
        
{\bf Behavioral:} \\[1mm]
\HS\TR[\BTS]{\Class\C{\fd[1]..}{\md[1].. }} 
    & =  \src{\Class \C {\fd[1]..}{\mdp[1].. } } \\    
    & \WHERE \HS\HS\HS \mdp[1] = \src{\Mdef\m\x\t\tp{\ep[1]}} ..\HS\HS \\   
    & \HS\HS\HS\HS\HS\HS\HS\HS\HS \md[1] = \Mdef\m\x\t\tp{\e[1]} ..\HS\HS 
    \HS\HS \ep[1] = \TRG[\BTS]{\e[1]}{\x:\t\,\this:\C} \\    


{\bf Concrete:} \\[1mm]
   
\HS\TR[\CTS]{\Class\C{\fd[1]..}{\md[1].. }} 
    & = \src{ \Class \C{ \fd[1]..}{\mdp[1].. \mdpp[1]..}} \\   
    & \WHERE \HS\HS\HS {\mdp[1]} = \src{\Mdef\m\x{{\t[1]}}{{\t[2]}}{\ep}} .. \\    
    & \HS\HS\HS\HS\HS\HS\HS\HS\HS \md[1] = \Mdef\m\x{\t[1]}{\t[2]}\e .. 
   \HS\HS \ep = \TAG[\CTS]{\e}{\this:\C\,\x:\t[1]}{\t[2]}~  ..\\
    & \HS\HS\HS\HS\HS\HS\HS\HS\HS {\mdpp[1]} = \src{\Mdef\m\x\any\any{\SubCast\any{\KCall\this\m{\SubCast{{\t[1]}}\x}{\t[1]}{\t[2]}}}} \\     
    & \HS\HS\HS\HS\HS\HS\HS\HS\HS\HS \HS\HS\HS\HS\HS\HS\HS\HS\HS\HS\HS \textbf{\IF} {\t[1]} $\neq$ \any \\    
    & \HS\HS\HS\HS\HS\HS\HS\HS\HS \HS\HS\HS\HS\HS\HS \src{empty}    
    \HS {\bf otherwise}  ..   
  \end{tabular}   \\[-2mm]
      
\hrulefill}
 \caption{Translations for classes.}     \label{fig:traclass}    
\end{figure}

\vspace{2mm}\noindent {\bf Optional.~} The optional approach provides no
correctness guarantees.  Retaining the surface type annotations through
translation would not preserve this semantics, so we erase them.  The
resulting class has all fields, all method arguments, and all return
values typed as \any.

\vspace{2mm}\noindent {\bf Transient.~} In the transient approach, ensure
that for any method call, the receiver does have a method with the
corresponding name. To encode this within the \kafka type system requires
replacing all of the argument and return types with \any. This translation
allows functions to be called under any type and to return values of any
type. Casts to the erased types are then effectively shallow structural
checks only.  As there is no
guarantee that fields contain values of their type,
the translation sets their type to \any.

\vspace{2mm}\noindent {\bf Behavioral.~} The behavioral approach guarantees
soundness by wrapping values that cross type-untyped boundaries. Methods
are preserved by the translation but bodies are translated.

\vspace{2mm}\noindent {\bf Concrete.~} The concrete approach ensures that
variables of non-\any types refer to subtypes of the given type. Each method
appearing in the original class is retained as such with its body
translated.  Moreover, all typed methods could be called from an untyped
context, so untyped variants are generated that guard the typed functions.
These variants perform subtype casts on their arguments to ensure that they
were given the right types, then call the guarded typed function.

\subsection{Expression Translation} 

To accommodate differences between the gradual typing semantics, we use two
different expression translation schemes. The first is a type-agnostic
one, used for the optional approach. $\TR[\OTS]\e$ denotes optional translation,
where \e is the target expression, and the result is a \kafka term. We use
this form to simplify the optional translation, as it is ambivalent about the
types of the expressions it is translating; the optional semantics simply
eliminates all of them.

The second translation form is type-aware, used for the three other
approaches. The type-aware translation has two forms, $\TRG[\SOMS]\e\Env$
and $\TAG[\SOMS]\e\Env\t$, inspired by work on bidirectional
type-checking~\cite{pierce:1998:local}.  The first form,
$\TRG[\SOMS]\e\Env$, is analogous to the synthetic case in bidirectional
type-checking.  It is used for expressions without any specific required
type.  The second form, $\TAG[\SOMS]\e\Env\t$, is used when \e must have
some type \t. Analogous to the analytic case of bidirectional type-checking,
this form applies when some enclosing expression has an expectation of the
type of \e. For example, it is used in translation of method arguments,
which must conform to the types of the arguments to the method. We refer to
this as assertive translation. These two forms allow us to identify where
consistency was needed to conclude the surface level typing judgment.

\begin{figure}[!b]\small  \hrulefill\\[2mm]
\begin{tabular}{llc@{\hspace{.25cm}}l@{\HS}l@{\HS}l}

{\bf Transient:}\\[1mm]
\HS \TAG[\TTS]\e\Env\t & = \src\ep &\WHERE
    & \TypeCk{\K,\Env}\e\tp
    & \EM{\K\vdash\tp\Sub\t}
    & \ep = \TRG[\TTS]\e\Env \\
\HS\TAG[\TTS]\e\Env\t &= \src{\SubCast\t\ep} &\WHERE
    & \TypeCk{\K,\Env}\e\tp 
    & \EM{\K\vdash \tp \not \Sub \t}
    & \EM{\ep = \TRG[\TTS]\e\Env} \\[2mm]
{\bf Behavioral:} \\ [1mm]
 \HS\TAG[\BTS]\e\Env\t & = \src\ep & \WHERE
    & \TypeCk{\K,\Env}\e\tp
    & \EM{\K\vdash \tp \Sub \t}
    & \ep = \TRG[\BTS]\e\Env\\
\HS\TAG[\BTS]\e\Env\t & = \src{\BehCast\t\ep} & \WHERE
    & \TypeCk{\K,\Env}\e\tp \HS 
    & \EM{\K\vdash \tp \not \Sub \t}
    & \ep = \TRG[\BTS]\e\Env \\[2mm]
{\bf Concrete:} \\[1mm]
\HS\TAG[\CTS]\e\Env\t &= \src\ep &\WHERE
    & \TypeCk{\K,\Env}\e\tp 
    & \EM{\K\vdash\tp \Sub \t} 
    & \ep = \TRG[\CTS]\e\Env\\
\HS\TAG[\CTS]\e\Env\t &= \src{\SubCast{\t}\ep} &\WHERE
    & \TypeCk{\K,\Env}\e\tp 
    & \EM{\K\vdash\tp \not\Sub \t}
    & \EM{\ep = \TRG[\CTS]\e\Env} 
\end{tabular}
\\

\hrulefill

\caption{Assertive translation.}\label{fig:trtype}
\end{figure}

The assertive translation of \figref{fig:trtype} is responsible for producing
well-typed terms by adding casts into expressions where static types differ.
The rules closely track the convertibility relation of the surface language.
Every type-driven translation has two cases. The first case is used when the
required type happens to be a supertype of the expression's actual type, in
which cast upcasting can happen implicitly  and no further action is required.
The second case handles typed-untyped boundaries, conversions to or from \any.
The concrete and transient approaches both use the subtype cast operator to
protect these boundaries, though the effective semantics are different; concrete
retains the types that transient erases, so subtype casts in transient check
structural compatibility (e.g. are all the needed methods present) alone
whereas concrete subtype casts check the entire object's types.
The behavioral approach instead inserts behavioral casts
at boundaries.

The translation of field access appears in \figref{fig:travar}.  The
optional translation only inserts a cast to \any in front of uses 
\this as a technicality required for statically typing terms. The
transient translation casts variables and fields to their statically
expected type, as their values may be of any type.  In transient, however,
subtype casts only check the structure of the types. The behavioral
translation and the concrete translation leave both types of access intact.

\begin{figure}[!h]\small\hrulefill\\
\begin{tabular}{@{}l@{\HS}l}
\\[-2mm]

\begin{tabular}{llc@{\hspace{.25cm}}l@{\HS}l@{\HS}l}

{ \bf Optional:} \\[2mm]
\HS\TR[\OTS]\x & = \src \x \\
\HS\TR[\OTS]\this & = \src{\SubCast\any\this} \\
\HS\TR[\OTS]{\FRead\f} & = \src{\FRead\f} \\
\\
\end{tabular}
&
\begin{tabular}{llc@{\hspace{.25cm}}l@{\HS}l@{\HS}l}
{ \bf Transient:}\\[2mm]
\HS\TRG[\TTS]\x\Env & = \src{\SubCast\t\x} & \WHERE & \TypeCk{\K,\Env}\x\t \\
\HS\TRG[\TTS]\this\Env & = \src\this \\
\HS\TRG[\TTS]{\FRead\f}\Env & = \src{\SubCast\t{\FRead\f}} & \WHERE & \TypeCk{\K,\Env}\this\C \HS \Ftype\f\t\In\App\K\C \\
\end{tabular}
\\
\begin{tabular}{llc@{\hspace{.25cm}}l@{\HS}l@{\HS}l}		
{ \bf Behavioral:} \\[2mm]
\HS\TRG[\BTS]\x\Env &= \src{\x} \\
\HS\TRG[\BTS]\this\Env &= \src{\this} \\
\HS\TRG[\BTS]{\FRead\f}\Env  &= \src{\FRead\f}
\end{tabular}
&
\begin{tabular}{llc@{\hspace{.25cm}}l@{\HS}l@{\HS}l}		
{\bf Concrete:}\\[2mm]
\HS\TRG[\CTS]{\x}\Env & = \src \x \\
\HS\TRG[\CTS]\this\Env &= \src{\this} \\
\HS\TRG[\CTS]{\FRead\f}\Env        & = \src{\FRead\f}
\HS\end{tabular}
\end{tabular}\\

\hrulefill
\caption{Translations variables and field access.}\label{fig:travar}
\end{figure}

The translation for assignment is shown in \figref{fig:trassn}.  All the
approaches translate the value only differing in the expected
type. Behavioral and concrete require that the result has the statically
known type, transient expects \any, and the optional semantics imposes no
type requirement whatsoever.

\begin{figure}[!h]\small
\hrulefill\\
\begin{tabular}{llc@{\hspace{.25cm}}l@{\HS}l@{\HS}l}\\[-1mm]

{\bf Optional:}\\[1mm]
\HS\TR[\OTS]{\FWrite\f\e} 
        & = \src{\FWrite\f\ep} &\WHERE&\ep=\TR[\OTS]\e\\[2mm]
{\bf Transient:}\\[1mm]
\HS\TRG[\TTS]{\FWrite\f\e}\Env & =  \src{{\FWrite\f\ep}} &\WHERE
        & \TypeCk{\K,\Env}\this\C
        & \Ftype\f\t\In\App\K\C 
	& \ep = \TAG[\TTS]\e\Env\any\\[2mm]
{\bf Behavioral:}\\ [1mm]
\HS\TRG[\BTS]{\FWrite\f\e}\Env &=  \src{\FWrite\f\ep} & \WHERE
	& \TypeCk{\K,\Env}{\this}\C
	& \Ftype\f\t\In\App\K\C 
	& \ep = \TAG[\BTS]\e\Env\t\\[2mm]
{\bf Concrete:}\\[1mm]
\HS\TRG[\CTS]{\FWrite\f\e}\Env     & = \src{\FWrite\f\ep} & \WHERE
	& \TypeCk{\K, \Env}\this\C
	& \Ftype\f\t\In\App\K\C
	& \ep = \TAG[\CTS]\e\Env{\t} 
\end{tabular}\\[-2mm]

\hrulefill\vspace{1mm}
\caption{Translations for assignment.}\label{fig:trassn}
\vspace{1mm}

\hrulefill\\
\begin{tabular}{llc@{\hspace{.25cm}}l@{\HS}l@{\HS}l}
\\[-2mm]
{\bf Optional:}\\[1mm]
\HS\TR[\OTS]{\New\C{\e[1]..}} & = \src{\SubCast\any{\New\C{\ep[1]..}}} &\WHERE 
	& \ep[1] = \TR[\OTS]{\e[1]} .. \\[2mm]
{\bf Transient:}\\[1mm]
\HS\TRG[\TTS]{\New\C{\e[1]..}}\Env &=  \src{\New\C{\ep[1]..}} &\WHERE 
	& \Ftype{\f[1]}{\t[1]}\In\App\K\C
	& \ep[1] = \TAG[\TTS]{\e[1]}\Env{\any} ~.. \\[2mm]
{\bf Behavioral:}\\ [1mm]
\HS\TRG[\BTS]{\New\C{\e[1]..}}\Env & = \src{\New\C{\ep[1]..}} &\WHERE 
	& \Ftype{\f[1]}{\t[1]}\In\App\K\C
	& \ep[1] = \TAG[\BTS]{\e[1]}\Env{\t[1]} ~..\\
{\bf Concrete:} \\[1mm]
\HS\TRG[\CTS]{\New\C{\e[1]..}}\Env &= \src{\New\C{\ep[1]..}}  &\WHERE
	& \Ftype{\f[1]}{\t[1]}\In\App\K\C
	& \ep[1] = \TAG[\CTS]{\e[1]}\Env{\t[1]} ..
\end{tabular}\\[-2mm]

\hrulefill\vspace{1mm}
\caption{Translations for object creation.}\label{fig:tranew}
\vspace{1mm}

\hrulefill\\
\\[-2mm]
\begin{tabular}{llc@{\hspace{.25cm}}l@{\HS}l@{\HS}l}
{\bf Optional:}\\[1mm]
\HS\TR[\OTS]{\Call{\e[1]}\m{\e[2]}} &= \src{\DynCall{\ep[1]}\m{\ep[2]}} &\WHERE 
    & \ep[1] = \TR[\OTS]{\e[1]} & \ep[2] = \TR[\OTS]{\e[2]} \\[2mm]
{\bf Transient:} \\[1mm]
\HS\TRG[\TTS]{\Call{\e[1]}\m{\e[2]}}\Env 
        & = \src{\DynCall{\ep[1]}\m{\ep[2]}} & \WHERE 
	& \TypeCk{\K,\Env}{\e[1]}\any 
	& \ep[1] = \TRG[\TTS]{\e[1]}\Env
	& \ep[2] = \TAG[\TTS]{\e[2]}\Env\any \\ 
\HS\TRG[\TTS]{\Call{\e[1]}\m{\e[2]}}\Env 
        & = \src{\SubCast{\D[2]}{\KCall{\ep[1]}\m{\ep[2]}\any\any}}
	& \WHERE
	& \TypeCk{\K,\Env}{\e[1]}\C  
	& \ep[1] = \TRG[\TTS]{\e[1]}\Env  
        & \ep[2] = \TAG[\TTS]{\e[2]}\Env{\any} \\
        & & & \multicolumn{2}{l}{\Mtype\m{\D[1]}{\D[2]}\In\App\K\C} \\[2mm]
{\bf Behavioral:}\\[1mm]
\HS\TRG[\BTS]{\Call{\e[1]}\m{\e[2]}}\Env 
        & = \src{\DynCall{\ep[1]}\m{\ep[2]}} & \WHERE
	&  \TypeCk{\K,\Env}{\e[1]}\any
	&  \ep[1] = \TRG[\BTS]{\e[1]}\Env
	&  \ep[2] = \TAG[\BTS]{\e[2]}\Env\any
\\
\HS\TRG[\BTS]{\Call{\e[1]}\m{\e[2]}}\Env & = \src{\KCall{\ep[1]}\m{\ep[2]}{\D[1]}{\D[2]}} & \WHERE 
	& \TypeCk{\K,\Env}{\e[1]}\C 
	& \ep[1] = \TRG[\BTS]{\e[1]}\Env
	& \ep[2] = \TAG[\BTS]{\e[2]}\Env{\D[1]}  \\
	& & &  \multicolumn{2}{l}{\Mtype\m{\D[1]}{\D[2]}\In\App\K\C} \\[2mm]
{\bf Concrete:}\\[1mm]
\HS\TRG[\CTS]{\Call{\e[1]}\m{\e[2]}}\Env 
        & = \src{\DynCall{\ep[1]}{\m}{\ep[2]}} & \WHERE 
        &  \TypeCk{\K,\Env}{\e[1]}\any 
        &  \ep[1]= \TRG[\CTS]{\e[1]}\Env 
        & \ep[2] = \TAG[\CTS]{\e[2]}\Env\any\\
\HS\TRG[\CTS]{\Call{\e[1]}\m{\e[2]}}\Env 
        & = \src{\KCall{\ep[1]}{\m}{\ep[2]}{\D[1]}{\D[2]}} 
	& \WHERE & \TypeCk{\K,\Env}{\e[1]}\C 
        &  \ep[1] = \TRG[\CTS]{\e[1]}\Env 
        &   \ep[2] = \TAG[\CTS]{\e[2]}\Env{\D[1]} \\ 
	& & & \multicolumn{2}{l}{\Mtype\m{\D[1]}{\D[2]}\In\App\K\C} &  \\
\end{tabular}\\
\hrule	\vspace{1mm}
\caption{Translations for function invocation.}\label{fig:trafuninv}
\end{figure}

The translation for object creation, shown in \figref{fig:tranew}, follows
the same reasoning. It inserts casts for each argument to be the required type
according to class translation.

The translations for invocation are shown in \figref{fig:trafuninv}.  The
optional approach translates all invocations to dynamic invocation, as it
cannot provide any static guarantee. In the concrete and behavioral
approaches, since the static types are retained, arguments must be asserted
to have the statically known type. In the transient semantics, the argument
type is ignored, so the argument to a statically typed method call is only
required to be of type \any, but the return type is checked.  In all of the
systems, if the type of the receiver is \any, dynamic invocation is used.

\newpage

\subsection{Example}

We illustrate the translation with the behavior of litmus program {\bf L3}.
The operational principle of {\bf L3} is that it creates a new object (an
instance of \C), then uses an untyped intermediate to represent it as type
\E. Type \E ascribes the wrong type for argument \x, substituting \D for the
correct type \C. 

\begin{figure}[!h]\small
\hrulefill\\
\\
\begin{tabular}{l}
{\bf Source:} \\[2mm]
\(
\begin{array}{l@{\,}l}
\Class{\xt F}{}{&\Mdef\m\x{\xt E}{\xt E}\x \HS\HS
    \Mdef\n\x\any\any{\Call\this\m\x}} \\
\end{array}
\) \\[2mm]
{\bf Optional:}\\[2mm]
\(
\begin{array}{l@{\,}l}
\Class{\xt F}{}{&\Mdef\m\x{\any}{\any}\x  \HS\HS
    \Mdef\n\x\any\any{\DynCall{(\SubCast\any\this)}\m\x}} 
\end{array}
\) \\[2mm]
{\bf Transient:}\\[2mm]
\(
\begin{array}{l@{\,}l}
\Class{\xt F}{}{
   &\Mdef\m\x\any\any{\SubCast{\xt E}{\x}; ~ \SubCast{\any}{\x} } 
    \HS\HS \Mdef\n\x\any\any{\SubCast{\any}{\x}\sspce 
   \SubCast{\any}{\SubCast{\xt E}{\KCall\this\m{\SubCast\any{\SubCast\any\x}}\any\any}}}} 
\end{array}
\)\\[2mm]
{\bf Behavioral:} \\[2mm]
\(
\begin{array}{l@{\,}l}
\Class{\xt F}{}{&\Mdef\m\x{\xt E}{\xt E}\x \HS\HS
      \Mdef\n\x\any\any{\BehCast\any{\KCall\this\m{\BehCast{\xt E}\x}{\xt E}{\xt E}}}} 
\end{array}
\) \\[2mm]
{\bf Concrete:} \\[2mm]
\(
\begin{array}{l@{\,}l}
\Class{\xt F}{}{&\Mdef\m\x{\xt E}{\xt E}\x  \HS\HS
       \Mdef\n\x\any\any{\SubCast\any{\KCall\this\m{\SubCast{\xt E}\x}{\xt E}{\xt E}}}} 
\end{array}
\) \\
\end{tabular}\vspace{2mm}\\
\hrule\vspace{4mm}

 \caption{Class translation for litmus test L3.} \label{fig:l3trans}
\end{figure}

Two of the gradual type systems notice this invalid type. Concrete errors on
{\bf L3} because \E is not a subtype of \C.  With behavioral, the unused
type ascription is saved as a wrapper and is enforced causing a run-time error.

While this reasoning provides an intuition, it provides few detail for which
we turn to our formalism.  We present the translation from the top, starting
with classes in \figref{fig:l3trans}.  The optional approach does no
checking whatsoever, and simply erases types. Transient also erases types,
but adds argument casts on method entry. In the case of \m, argument \x is
checked to be of type \E, as the translation of type \E does not include
types no type error will be reported.  Behavioral retains typed methods but
adds behavioral casts on untyped methods.  The concrete semantics retains
typed methods, and adds a subtype cast when a variable of type \any is passed
to a method that expects and \E.

\begin{figure}[!h]\small
\hrulefill\\
\\
\begin{tabular}{rl}
  \multicolumn{2}{l}{\begin{tabular}{l}
{\bf Source:}\\[2mm]
\(\begin{array}{l@{\,}l} 
\Class{\xt E}{}{&\Mdef\m\x{\xt D}{\xt D}\x } \\
\end{array}\) 
\end{tabular}}
\\[2mm]\\
\begin{tabular}{@{}l}
{\bf Optional:}\\[2mm]
\(\begin{array}{l@{\,}l}
\Class{\xt E}{}{&\Mdef\m\x{\any}{\any}\x } \\
\end{array}\) 
\end{tabular}&
\begin{tabular}{l}
{\bf Transient:}\\[2mm]
\(\begin{array}{l@{\,}l}
\Class{\xt E}{}{&\Mdef\m\x\any\any{\SubCast{\xt E}\x ; ~ \SubCast{\any}{\x}}} \\
\end{array}\)
\end{tabular}\\\\
\begin{tabular}{l}
{\bf Behavioral:}\\[2mm]
\(\begin{array}{l@{\,}l}
\Class{\xt E}{}{&\Mdef\m\x{\xt E}{\xt E}\x} \\
\end{array}\) 
\end{tabular} &
\begin{tabular}{l}
{\bf Concrete:}\\[2mm]
\(\begin{array}{l@{\,}l}
\Class{\xt E}{}{&\Mdef\m\x{\xt E}{\xt E}\x} \\
\end{array}\) 
\end{tabular}\\
\end{tabular}\vspace{2mm}\\
\hrule\vspace{4mm}
  
 \caption{Translation of \xt{E} in litmus test L3.}  \label{fig:l3etrans}
\end{figure}

\figref{fig:l3etrans} presents the translation of class \E.  For the
transient semantics, when \x is cast to \E, all of the types on \E are
erased. Casting to \E is tantamount to asking for the existence of the
method \m. In contrast, the concrete semantics retains the types of \m. A
cast to \E is equivalent to checking if a method \m that takes and returns
an \E exists.  This comes at the cost of the ability to migrate between
untyped and typed code. Suppose that both the optional and concrete versions
of \E existed, under a different name {\xt F}. In that program, only the
concrete version of \E could be used with the concrete version of {\xt
  F}. Despite implementing the same behavior, Behavioral uses the same
representation for \E as concrete. The behavioral cast allows to use any
value that behaves like an \E.

To examine the operation of the behavioral cast in more detail,
\figref{fig:behex} depicts the wrapper classes generated at the cast
from \C to \any and from it to \xt E.  Class $\C_1$ takes an instance of \C
and makes it safe against use as \any. In behavioral, no typed invocations
can be made on a value that was cast to \any (and not cast to some type
somewhere); only untyped invocations are allowed. As a result, the wrapper
need only generate an untyped version of \C's method \a, which calls the
underlying \C instance's \a (adding suitable casts).  The second wrapper
class $\C_2$ takes the $\C_1$ wrapper and casts it back to \E. This wrapper
takes the untyped implementation of \a and wraps it again, calling it with
an argument cast to \any and casting the return to \D.

\begin{figure}[h!]\hrulefill\vspace{2mm}

\begin{tabularx}{\textwidth}{XX}
\Class\C{}{\Mdef{\xt{a}}\x\C\C\x} & \Class{\xt E}{}{\Mdef{\xt{a}}\x\D\D\x}
\end{tabularx}

\vspace{-4mm}
\begin{align*}
\Class{\C_1}{\HS&\that : \C}{&\Mdef{\xt{a}}\x\any\any{\BehCast\any{\KCall{\this.\that}{\xt{a}}{\BehCast\C\x}\C\C}}} \\
\Class{\C_2}{\HS &\that : \C_1}{&\Mdef{\xt{a}}\x\D\D{\BehCast\D{\KCall{\this.\that}{\xt{a}}{\BehCast\any\x}\any\any}}}
\end{align*}
\vspace{-8mm}

\hrulefill
\caption{Behavioral wrappers.}\label{fig:behex}
\end{figure}

\subsection{Discussion}

These translations explicit the enforcement machinery of each of the four
approaches.  Programs can get stuck at dynamic invocation and
casts. Inspecting where these are inserted gives a precise account of what
constitutes an error in each gradual type system.

Our account of the behavioral approach matches its implementation in Typed
Racket. However, one could imagine a slightly less restrictive implementation,
one which does not have a check for method names at wrapper creation.  That
check is pragmatic but perhaps too strict --- it will rule out programs that
may be fine just because a method is missing. One could have a wrapper that
simply reports an error if a missing method is called.

Performance is a perennial worry for implementers of gradual type systems.
It is difficult to guess how a highly optimizing language
implementation will perform, as these implementations are likely to optimize
away the majority of the casts and dynamic dispatches. Consider the progress
in the performance of Typed Racket reported in the
literature~\cite{popl16,OnlyMostly}.  What we can tell by looking at the
translations is that with optional there is no obvious benefit or cost to
having type annotations. Transient has checks on reads, which are common,
and typed function calls. Furthermore, those checks are needed even if the
entire program is typed. Both concrete and behavioral can benefit from type
information in typed code.  The difference is that the cost of boundary
crossing are low in the concrete approach, as it uses a subtype check whereas
behavioral requires allocation of a wrapper. Wrappers 
may also complicate the task of devirtualization and unboxing.


\section{Conclusion}

This paper introduced \kafka, a framework for comparing the design of
gradual type systems for object-oriented languages. Our approach is to provide
translations with different gradual semantics from a common surface language
into \kafka. These translations highlight the different run-time enforcement
strategies deployed by the languages under study. The differences between
gradual type systems are highlighted explicitly by the observable differences
of their behavior in our litmus tests, demonstrating how there is no consensus
on the meaning of error.  These litmus tests motivated the need to have a
common framework to explore the design space.

\kafka demonstrates that to express the different gradual approaches, one
needs a calculus with two casts (structural and behavioral), two
invocation forms (dynamic and static), the ability to extend the
class table at run-time, and wrappers that expose their underlying
unwrapped methods.  We provide a mechanized proof of soundness for \kafka
that includes run-time class generation.  We also demonstrate that \kafka
can be straightforwardly implemented on top of a stock virtual machine.

A open question for gradual type system designers is performance of the
resulting implementation. Performance remains a major obstacle to adoption
of approaches that attempt to provide soundness guarantees.  Under the
optional approach, types are removed by the translation; as a result,
performance will be identical to that of untyped code.  The transient
approach checks types at uses, so the act of adding types to a program
introduces more casts and may slow the program down (even in fully typed code). 
In contrast, the behavioral approach avoids casts in
typed code. The price it pays for this soundness, however, is that heavyweight
wrappers inserted at typed-untyped boundaries.  Lastly, the concrete
semantics is also sound and has low overheads, but comes at a cost in
expressiveness and ability to migrate from untyped to typed.

Going forward, there are several issues we wish to investigate.  We do not
envision that supporting nominal subtyping within \kafka will pose problems,
it would only take adding a nominal cast and changing the definition of
classes. Then nominal and structural could coexist. A more challenging
question is how to handle the intricate semantics of Monotonic Reticulated
Python. For these we would need a somewhat more powerful cast operation.
Rather than building each new cast into the calculus itself, it would be
interesting to axiomatize the correctness requirements for a cast and let
users define their own cast semantics. The goal would be to have a
collection of user defined pluggable casts within a single framework.


==> FrontBackmatter/Colophon.tex <==
\pagestyle{empty}

\hfill

\vfill


\pdfbookmark[0]{Colophon}{colophon}
\section*{Colophon}
This document was typeset using the typographical look-and-feel \texttt{classicthesis} developed by Andr\'e Miede. 
The style was inspired by Robert Bringhurst's seminal book on typography ``\emph{The Elements of Typographic Style}''. 
\texttt{classicthesis} is available for both \LaTeX\ and \mLyX: 
\begin{center}
\url{https://bitbucket.org/amiede/classicthesis/}
\end{center}
Happy users of \texttt{classicthesis} usually send a real postcard to the author, a collection of postcards received so far is featured here: 
\begin{center}
\url{http://postcards.miede.de/}
\end{center}
 
\bigskip

\noindent\finalVersionString

%Hermann Zapf's \emph{Palatino} and \emph{Euler} type faces (Type~1 PostScript fonts \emph{URW
%Palladio L} and \emph{FPL}) are used. The ``typewriter'' text is typeset in \emph{Bera Mono}, 
%originally developed by Bitstream, Inc. as ``Bitstream Vera''. (Type~1 PostScript fonts were made 
%available by Malte Rosenau and
%Ulrich Dirr.)

%\paragraph{note:} The custom size of the textblock was calculated
%using the directions given by Mr. Bringhurst (pages 26--29 and
%175/176). 10~pt Palatino needs  133.21~pt for the string
%``abcdefghijklmnopqrstuvwxyz''. This yields a good line length between
%24--26~pc (288--312~pt). Using a ``\emph{double square textblock}''
%with a 1:2 ratio this results in a textblock of 312:624~pt (which
%includes the headline in this design). A good alternative would be the
%``\emph{golden section textblock}'' with a ratio of 1:1.62, here
%312:505.44~pt. For comparison, \texttt{DIV9} of the \texttt{typearea}
%package results in a line length of 389~pt (32.4~pc), which is by far
%too long. However, this information will only be of interest for
%hardcore pseudo-typographers like me.%
%
%To make your own calculations, use the following commands and look up
%the corresponding lengths in the book:
%\begin{verbatim}
%    \settowidth{\abcd}{abcdefghijklmnopqrstuvwxyz}
%    \the\abcd\ % prints the value of the length
%\end{verbatim}
%Please see the file \texttt{classicthesis.sty} for some precalculated 
%values for Palatino and Minion.
%
%    \settowidth{\abcd}{abcdefghijklmnopqrstuvwxyz}
%    \the\abcd\ % prints the value of the length






==> FrontBackmatter/Declaration.tex <==
%*******************************************************
% Declaration
%*******************************************************
\refstepcounter{dummy}
\pdfbookmark[0]{Declaration}{declaration}
\chapter*{Declaration}
\thispagestyle{empty}
Put your declaration here.
\bigskip
 
\noindent\textit{\myLocation, \myTime}

\smallskip

\begin{flushright}
    \begin{tabular}{m{5cm}}
        \\ \hline
        \centering\myName \\
    \end{tabular}
\end{flushright}


==> FrontBackmatter/Dedication.tex <==
%*******************************************************
% Dedication
%*******************************************************
\thispagestyle{empty}
%\phantomsection 
\refstepcounter{dummy}
\pdfbookmark[1]{Dedication}{Dedication}

\vspace*{3cm}

\begin{center}
    To my loving parents for all of their love and support.
\end{center}

==> FrontBackmatter/Publications.tex <==
%*******************************************************
% Publications
%*******************************************************
%\pdfbookmark[1]{Publications}{publications}
%\chapter*{Publications}\graffito{This is just an early --~and currently ugly~-- test!}
%This might come in handy for PhD theses: some ideas and figures have appeared previously in the following publications:

%\noindent Put your publications from the thesis here. The packages \texttt{multibib} or \texttt{bibtopic} etc. can be used to handle multiple different bibliographies in your document.

%\begin{refsection}[ownpubs]
%    \small
%    \nocite{*} % is local to to the enclosing refsection
%    \printbibliography[heading=none]
%\end{refsection}

%\emph{Attention}: This requires a separate run of \texttt{bibtex} for your \texttt{refsection}, \eg, \texttt{ClassicThesis1-blx} for this file. You might also use \texttt{biber} as the backend for \texttt{biblatex}. See also \url{http://tex.stackexchange.com/questions/128196/problem-with-refsection}.

==> FrontBackmatter/Titleback.tex <==
\thispagestyle{empty}

\hfill

\vfill

\noindent\myName: \textit{\myTitle,} \mySubtitle, %\myDegree, 
\textcopyright\ \myTime

%\bigskip
%
%\noindent\spacedlowsmallcaps{Supervisors}: \\
%\myProf \\
%\myOtherProf \\ 
%\mySupervisor
%
%\medskip
%
%\noindent\spacedlowsmallcaps{Location}: \\
%\myLocation
%
%\medskip
%
%\noindent\spacedlowsmallcaps{Time Frame}: \\
%\myTime

